NeuroDB: A Neural Network Framework for Answering Range Aggregate Queries and Beyond

Range aggregate queries (RAQs) are an integral part of many real-world applications, where, often, fast and approximate answers for the queries are desired. Recent work has studied answering RAQs using machine learning models, where a model of the data is learned to answer the queries. However, such modelling choices fail to utilize any query specific information. To capture such information, we observe that RAQs can be represented by query functions, which are functions that take a query instance (i.e., a specific RAQ) as an input and output its corresponding answer. Using this representation, we formulate the problem of learning to approximate the query function, and propose NeuroDB, a query specialized neural network framework, that answers RAQs efficiently. NeuroDB is query-type agnostic (i.e., it does not make any assumption about the underlying query type) and our observation that queries can be represented by functions is not specific to RAQs. Thus, we investigate whether NeuroDB can be used for other query types, by applying it to distance to nearest neighbour queries. We experimentally show that NeuroDB outperforms the state-of-the-art for this query type, often by orders of magnitude. Moreover, the same neural network architecture as for RAQs is used, bringing to light the possibility of using a generic framework to answer any query type efficiently.

==> Introduction_old.tex <==
\section{Introduction}
Range aggregate queries are a building block of various real world applications, from calculating total profit over a period from sales records to calculating average time spent by users in an area in a geo-spatial database. Often, exact answers are not required and an approximate but fast answer is preferred. For instance, an exact answer to the range aggregate query of calculating average pollution level for different time periods and regions for city planing \cite{ma2019dbest} may take too long due to large volume of data, but an approximate answer may be as valuable. In such scenarios, there exists a time/space/accuracy trade-off, where algorithms can sacrifice accuracy for time or space. 

Answering range aggregate queries has been studied for decades in the area of approximate query processing \cite{chaudhuri2017approximate}, where the goal is to improve upon the time/space/accuracy trade-off. Broadly speaking, the methods can be divided into sampling-based methods \cite{hellerstein1997online, agarwal2013blinkdb, chaudhuri2007optimized, park2018verdictdb} 
and model-based methods \cite{graham2012synopses, schmidt2002propolyne, ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. Sampling-based methods randomly sample a set of points from the database according to a sampling strategy, % (e.g., uniform sampling, \cite{hellerstein1997online}, stratified sampling \cite{chaudhuri2007optimized, park2018verdictdb})
and answer the queries based on the samples.  Model-based methods develop a model of the data that is used to answer queries. The models can be of the form of histograms, wavelets, data sketches (see \cite{graham2012synopses} for a survey) or, more recently, regression and density based models \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. %Generally, the model-based approached follow two steps. First, a model of the data is created. Then, a method is proposed to use these data models to answer the queries. 
Recent work \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}  has used machine learning and different modeling choices have been proposed to learn the data distribution. These studies show that modelling the data using machine learning techniques improves the accuracy over existing sampling-based techniques.

While the machine learning models have been successful, the modelling choices can be improved substantially. We first discuss three design principles that we utilize to improve upon the state-of-the-art in this paper. 

\noindent\textbf{Not All Queries Are Equal}. In real-world databases, certain queries are far more common than others. For instance, in a geo-spatial dataset containing latitude and longitude of visits of individuals to a location, together with the visit duration, a common range aggregate query consists of a range predicate on the location with the average aggregation function on the visit duration (while, e.g., the query of average latitude given a visit duration predicate may not make any semantic sense). For such frequent queries, speeding up the computation can improve the performance of the system.  However, the query distribution is ignored in recent machine learning methods \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb} for answering range aggregate queries. %Existing work misses the opportunity to learn information about the common queries that can help answering them faster.

\noindent\textbf{Query Specialization}. Modelling the data, as done in \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}, does not use any query specific information in learning. The model learnt is oblivious to the queries being asked. An alternative to modelling the data and using that model to answer all different queries is to learn specialized models for specific queries. Using query specialized models, different models are learned to answer different queries. For instance, in the geo-spatial dataset example, a model can be learned that is trained to answer queries with a range predicate on location and average aggregation function on visit duration.  Intuitively, a model specialized for a specific query (e.g., for specific range predicates and aggregation function and attribute) can answer the query more accurately and faster than a single model of the entire data, because the model only needs to learn the relevant information from the data to that particular query. Furthermore, given that in real-world datasets, not all possible queries are typically asked (or are meaningful, as mentioned in the paragraph above) the learned model can include less redundant information compared with the data. Nevertheless, multiple query-specialized models may consume more space than a single data model, but, even in that case, the space consumption is traded for better query time and accuracy, extending the set of achievable time/space/accuracy trade-offs. 

\noindent\textbf{Queries Are Functions}. Finally, we observe that range aggregate queries can be thought of as functions that can be approximated. This observation allows us to learn a specialized model, trained to answer a specific range aggregate query. Particularly, a \textit{query type} (or a \textit{query function}) on a database defines what the output should be for a \textit{query instance}\footnote{We use \textit{query instance} and \textit{query function} terminologies to distinguish between a particular query input (instance) and the general relationship between query inputs and their corresponding outputs (function).} on the database and can be seen as a function mapping the \textit{query space} to some \textit{output space}. For instance, in the geo-spatial database example, the input to the function is a range predicate and the output is a value in $R$. To answer this query type, we can learn a model (or function approximator) that approximates the specific query function, where the model takes as input a range predicate and outputs a real number. Different models can be trained for different query functions, each optimized for the specific query. %An approximation algorithms can be seen as functions approximating the query function, or, in other words, as \textit{function approximators}. 



%Answering database queries fast, with low storage cost and high accuracy are important performance goals in a database system. A general trade-off exists between these metrics, e.g., query time can be improved by increasing space consumption or sacrificing accuracy. In some applications, exact answers are not required and an approximate but fast answer is preferred. For instance an exact answer to the \textit{range aggregate query} of calculating average pollution level for different time periods and regions for city planing \cite{ma2019dbest} may take too long due to large volume of data, but an approximate answer may be as valuable. Many other scenarios where approximate answers to queries are acceptable are considered in the literature \cite{chaudhuri2017approximate}. Another example is distance-based outlier detection \cite{chandola2009anomaly} on a video stream, or selecting video frames for training a vision model \cite{settles2009active, fujii1999selective} from a video stream that requires algorithms that compute  \textit{distance to the $k$-th nearest neighbour} of the frames of a video stream over an existing database of images on the fly. The need for fast answers is often aggravated by the limitations of the device performing the computation. IoT and edge devices with limited processing/storage capacity are being utilized more often to capture videos and perform these operations \cite{qian2019active, Yang2018active}. Accuracy can be sacrificed for faster query response time to allow for processing of more video frames.  We primarily focus on range aggregate queries and distance to nearest neighbour queries which are two important underlying query types for which approximate answers are acceptable.

%\noindent\textbf{Grand Vision}. Another less-studied aspect of designing algorithms for different queries is the limitations and downsides of manually designed algorithms. In addition to the human time spent on designing efficient algorithms which could be saved, distribution of the data points and the query points are not fully exploited and the set of potential solutions is limited to human imagination and throughput. An automated framework that can efficiently answer range aggregate queries and distance to nearest neighbour queries,  and other, potentially new or application specific, types of queries is ideal. \textit{This paper is our first step towards the ultimate goal of devising a system that can automatically search an algorithm space to find algorithms with better time/space/accuracy trade-offs for different query types}, where an algorithm space is a set of potential algorithms that answer a query. 


%the human time spent on designing efficient algorithms, and the limitations of manually designed algorithms. Nearest neighbour queries are studied separately \cite{friedman1975algorithm, guan1992equal, bei1985improvement} from range aggregate queries \cite{graham2012synopses, hellerstein1997online, park2018verdictdb, ma2019dbest}, and several customized \textit{query-specific} algorithms have been developed to answer them efficiently. The large space of potential algorithms is manually explored by human experts to improve upon time/space/accuracy of the algorithms for different query types. However, no automated solution has been studied that can be applied to different query types. 

%\noindent\textbf{First Step}. Our first step towards that goal, presented in this paper, consists of

%We approach the problem by designing a framework that can learn an algorithm for one query type, namely, range aggregate queries, and showing that the same framework can be used to learn an algorithm for another query type, namely distance to the $k$-th nearest neighbour query, while outperforming the stat-of-the-art for both of them. Although an algorithm outperforming the state-of the-art in either of the two query types is significant on its own, our goal in this paper is to show that a learned framework can not only be useful for a specific query type, but can be generalizable to multiple query types (specifically query types that are traditionally studied separately, e.g., nearest neighbour queries and range aggregate queries). As such, it can improve the performance of a system while also saving time when designing it.

%To that end, in this paper, we make the observation that queries can be thought of as functions that can be approximated. This allows us to formulate a learning task, i.e., to learn a model, to answer a query. To be specific, a  \textit{query type} (or a \textit{query function}) on a database defines what the output should be for a \textit{query instance}\footnote{We use \textit{query instance} and \textit{query function} terminologies to distinguish between a particular query input (instance) and the general relationship between query inputs and their corresponding outputs (function).} on the database and can be seen as a function mapping the \textit{query space} to some \textit{output space} (e.g., for the nearest neighbour query on a $d$-dimensional database, query space is all the points in $R^d$ and output space is all the points in the database). Algorithms can be seen as functions approximating the query function, or, in other words, as \textit{function approximators}. This observation, generalizes ``Indexes are models'' of \cite{kraska2018case} to \textit{queries are functions that can be approximated}. %In \cite{kraska2018case}, traditional B-tree \cite{bayer2002organization} is replaced by a learned index. Our work can be seen as a generalization of their idea, where any query function can be replaced by a learned function approximated. 
%Using this terminology, where any algorithm is seen as a function approximating a query function\footnote{the approximation error is zero in many cases, e.g. for B-trees.}, we can say that a traditional B-tree \cite{bayer2002organization} as well as RMI \cite{kraska2018case} approximate an index query function, nearest neighbour query function can be approximated by combinatorial methods such as \cite{friedman1975algorithm, guan1992equal, bei1985improvement} and range aggregate query function by \cite{graham2012synopses, hellerstein1997online, park2018verdictdb}. 

\subsection{NeuroDB for Range Aggregate Queries}
We propose a novel framework, called \textit{Neural Databases} (NeuroDB), to efficiently answer range aggregate queries. By viewing database queries as functions, we propose a neural network framework that can approximate the query function well. Specifically, for a database, we consider range aggregate query functions of interest for which efficient answers are desired, e.g., the query of average visit duration for a particular location. Then, for each such query function, during a pre-processing step, NeuroDB learns a function approximator (or model) to approximate the query function. In this step, NeuroDB uses solved query instances from a known algorithm to train a model that specifically answers a particular query type well. The model takes the query instance as an input and outputs an answer, and the training objective is to optimize the model so that its answer is as close to ground truth as possible. Finally, at test time, NeuroDB uses the model to answer the queries efficiently, eliminating both the database and the algorithm it learned from.

We use neural networks as our function approximator. Neural networks can learn patterns in the real-world data and the relationship between query input and output, which means small models can answer queries well. They can be trained for specific query distributions, which allows more accurate modeling for the distribution and avoiding redundancies. In fact, NeuroDB can be seen as an approximate result materialization technique, where regions with higher probability in the query space are materialized more accurately. Furthermore, neural networks' architecture can be adjusted to learn complex queries and thus they can be applied to different domains with varying difficulty. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction. %Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section
%The neural network then can be used to replace the database for answering the queries. Our framework is simple and query-type agnostic, that is, it makes no assumption about the query type learned, and yet can provide orders of magnitude performance gains for the specific queries. We use neural networks to be able to capture the complex relationships that can exist between query inputs and outputs. 
However, designing a neural network architecture that can be easily trained, can answer the queries fast and accurately, and can scale with dimensionality and data size is not straightforward. We propose a novel architecture that achieves all of these objectives. 


Overall, NeuroDB offers significant improvements over the state-of-the-art query processing algorithms in multiple aspects. First, we experimentally observed that NeuroDB can answer queries multiple orders of magnitude faster than state-of-the-art and with better accuracy. Thus, in traditional data management systems, NeuroDB can be an addition to the query processing engine and can considerably improve the performance of range aggregate queries. A default query processing engine can answer queries for which NeuroDB is not trained while NeuroDB can be trained for common range aggregate queries, providing substantial improvements for the performance of the system. Furthermore, NeuroDB trained for a specific query is typically much smaller than data size, while the model learned can be used to answer the query it was trained for without accessing the data. This can be beneficial for applications requiring efficient release and storage of data. For instance, location data aggregators (e.g., SafeGraph \cite{safegraph}) can train a NeuroDB to answer the average visit duration query, and release it to interested parties instead of the entire dataset, which can improve the storage, transmission and query processing costs for all parties involved. 

%From another perspective, NeuroDB can be seen as an approximate result materialization technique that takes advantage of query and data distribution to minimize the approximation error. Roughly speaking, regions with higher probability in the query space are materialized more accurately, allowing the framework to perform well for high-dimensional data such as images where queries can be seen as belonging to low dimensional manifolds \cite{roweis2000nonlinear, chen2018sparse}. Intuitively, NeuroDB can be thought of as \textit{memorizing the data points} in the model weights. Although no general guarantee exists that this memorization should take less space than the actual data, in practice, we observe that due to the existence of patterns in the data and the relationship between query input and output, NeuroDB can answer queries by only taking up a fraction of the data size (and without the need to access the database). We note that this is different from merely \textit{memorizing or caching the answers to query points} in the training set, as we experimentally show that NeuroDB learns generalizable patterns between query input and output.

%Overall, in a database system, the choice of what range aggregate queries NeuroDB should be trained to answer is akin to the question of which attributes should be indexed.   


\subsection{Beyond Range Aggregate Queries}
Our observation that queries are functions that can be approximated is not specific to range aggregate queries, and is in fact true for any query type. Considering such representation opens the path for using learned function approximators for answering different database query types. In doing so, an important open question is to understand which function approximators are useful for which query types. 

We take the first step in studying this problem by applying NeuroDB to one more query type. This is possible because NeuroDB framework is query-type agnostic, that is, it does not make assumptions about the query type during training% and only requires solved instances of the query
. We considered two variants of $k$-th nearest neighbour queries. First, we considered $k$-th nearest neighbour queries ($k$-NN), which can be seen as functions that take a $d$-dimensional point as an input, where $d$ is the dimensionality of the database, and output another $d$-dimensional point. Applying NeuroDB to this query type, we experimentally observed that answering such a query requires very large neural networks, which does not provide any benefit in terms of query or storage cost compared with existing methods. Second, we considered the \textit{distance to} $k$-th nearest neighbour query, where the query answer is the distance to and not the actual point in the database. This query is a function that takes a $d$-dimensional query point as an input and outputs a real number. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (for instance, it can be used as a diversity score for selecting samples for training a model) or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. 

We observed that NeuroDB is able to answer distance to $k$-NN queries orders of magnitude faster than state-of-the-art, while only taking space that is a small fraction of data size. NeuroDB achieves this because it answers distance to $k$-NN queries without calculating any distances or finding any of the neighbours at query time. Contrasting this with existing methods that need to find the $k$-th nearest neighbour to calculate distance to $k$-th nearest neighbour shows another advantage of NeuroDB, where it can provide answers for specific queries without unnecessary precomputations. Furthermore, NeuroDB avoids curse of dimensionaity by utilizing the query distribution. For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all potential queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because the space of potential queries can be a small proportion of the total high dimensional space (e.g. for images). %This is in contrast to .  (e.g., finding the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. %without Although distance to $k$-NN queries is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

Overall, we conjecture that NeuroDB is useful for queries that are similar to range aggregate queries and distance to $k$-th nearest neighbour queries, where the answer to the queries is a numerical statistic calculated over the database. We consider studying this conjecture to be an interesting future research direction, where a generic framework can be used to answer multiple different query types. This paper is a first step in that direction, where a framework designed for range aggregate queries is shown to also efficiently answer distance to the $k$-th nearest neighbour queries and outperform the stat-of-the-art for both of them. Although NeuroDB outperforming the state-of the-art in either of the two query types is significant on its own, this paper also sheds light on the possibility that a learned framework can not only be useful for a specific query type, but can be generalizable to multiple query types (specifically query types that are traditionally studied separately, e.g., nearest neighbour queries and range aggregate queries). As such, it can improve the performance of a system while also saving time when designing it.


%The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%Searching the algorithm space translates into searching for good parameters of (or, in other words, learning) a function approximator. In this paper, as an initial attempt, we restrict the algorithm space to the set of parameters of a neural network because it can be searched efficiently. Therefore, we formalize the problem of using learned function approximators to answer database queries and show that, for the specific query types of distance to nearest neighbour query and range aggregate query, a learned neural network can provide better time/space/accuracy trade-offs than existing methods in practice. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction.%Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section


%Although the NeuroDB framework is query-type agnostic, and as such, can be applied to any query type, in this paper, we only show that it specifically provides orders of magnitude improvement for range aggregate queries and distance to nearest neighbour query. We do not make any claim about its efficiency for other query type. However, due to its good performance for the considered query types, we conjecture that NeuroDB can also be applied to other query types efficiently, but we leave studying this claim for the future work. Nevertheless, both queries considered in this paper are important building blocks of many real-world systems. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (for instance, it can be used as a diversity score for selecting samples for training a model) or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. Although it is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

%\noindent\textbf{NeuroDB vs. Combinatorial Methods}. To contrast NeuroDB with existing combinatorial methods, we note that (1) NeuroDB avoids curse of dimensionaity by utilizing the query distribution. For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all potential queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because the space of potential queries can be a small proportion of the total high dimensional space (e.g. for images). (2) NeuroDB can provide answers for specific queries without unnecessary precomputations. For instance, a model can be trained to find the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. 
%(3) Parallelization of NeuroDB is the problem of performing a forward pass of a neural network in parallel, is a well-studied problem [XX] and does not depend on the query type. 
%(3) NeuroDB uses query and data distribution to learn patterns that allow for answering queries faster. (4) The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%\noindent\textbf{NeuroDB vs. Machine Learning Methods}. Machine learning methods have been used to solve various combinatorial problems such as TSP, Max cut, etc \cite{li2018combinatorial, khalil2017learning, nazari2018reinforcement}. This paper extends those works to answering generic database queries using neural networks. Answering specific database queries using machine learning has been studied in the literature, such as for indexing \cite{kraska2018case, galakatos2018tree, ding2019alex} and specific aggregate queries \cite{hilprecht2019deepdb, ma2019dbest}. These methods have shown promise in the area they have been applied to, with their success being attributed to the ability of the models to learn and utilize the data and/or query distributions. The main observation in these bodies of work is that a certain database operation (e.g. getting the location a record is stored  for the case of indexing in \cite{kraska2018case}) can be replaced by a learned model. In this paper, we observe the overarching idea that, in fact, answering \textit{any} query can be done by a model, since any query is a function that can be approximated. Using this observation, we show that small, multi-layer neural networks can efficiently and accurately answer range aggregate queries and distance to nearest neighbour queries, improving on the modeling choices of the previous work and the state-of-the-art in the studied query types. %In this respect, our work can be seen as a generalization of the recent work in this area. The advantage in our framework is that it can be applied to different query types. %. However, no framework has been proposed that is able to answer different query types, i.e., both nearest neighbour and range aggregate queries efficiently. Furthermore the proposed techniques use basic regression models [X], while we show how the expressive power of multi-layer neural networks can be utilized.


\subsection{Contributions and Roadmap}

In this paper, we 

\begin{itemize}
        \item Formulate the problem of learning range aggregate queries with function approximators (Sec. \ref{sec:def}); 
        \item Propose the first neural network framework to answer range aggregate queries efficiently  (Sec. \ref{sec:NeuroDB}); and
        \item Show that the same framework can answer distance to nearest neighbour queries (Sec. \ref{sec:NN}).
        \item Our experiments show that
        \begin{enumerate}
            \item {NeuroDB} enjoys orders of magnitude gain in query time and provide better accuracy over state-of-the-art for answering range aggregate queries using real-world, TPC-benchmark and synthetic datasets (Sec.~\ref{sec:exp:rang_agg}); and
            \item The same architecture can be used to answer distance to nearest neighbour query with orders of magnitude gain in query time over state-of-the-art and optimal algorithms on real datasets. NeuroDB's query time is not affected by $k$ and only marginally impacted by data size and dimensionality (Sec. \ref{sec:exp:dist_NN}).
            %\item As a byproduct, we show that {NeuroDB} can learn patterns in the data, and thus is useful for feature learning or when there is missing data (Sec. \ref{sec:exp:NN}).  
        \end{enumerate}

\end{itemize}

We discuss the related work in Sec. \ref{sec:related_work} and further discuss the potentials and limitations of the proposed framework in Sec. \ref{sec:conclusion}. 

%Thus, our method is not applicable for NP-hard queries where collecting samples is difficult. 

%State the problem we're trying to solve: fast solution/not a lot of updates/low dimensional answer. Other examples of low dimensional query

\if 0

\begin{itemize}
    \item \textbf{Motivation}
    \begin{enumerate}
        \item Need for fast query processing, can sacrifice accuracy
        \begin{itemize}
        \item Running Examples: 
        \item (Distance to nearest neighbour query): distance-based outlier detection in video streams, or selecting video frames that are different enough from current samples for training. Want to analyze fast enough to process the stream on the fly
        \item (Range aggregate queries): Calculating avg. pollution level over time and regions for city planing \cite{ma2019dbest}. Large dataset, so exact solution takes too long, but error is acceptable
        \end{itemize}
        \item A lot of Human time is spent on designing efficient algorithms to answer queries
        \begin{itemize}
            \item Example: Different algorithms are designed for answering nearest neighbour queries, range aggregate queries, skyline queries, etc. 
            \item The algorithms are specific to queries
            \item So need to spend a lot of time designing new algorithms for new queries 
        \end{itemize}
    \end{enumerate}
        \item \textbf{Existing Solutions}
        \begin{itemize}
            \item Combinatorial Methods: Calculate answers by an algorithm that accesses the data
            \begin{itemize}
                \item Curse of dimensionality
                \begin{itemize}
                    \item Performance degrades with dimensionality
                    \item Neural network based dimensionality reduction methods are often used
                \end{itemize}
                \item Unnecessary calculations
                \begin{itemize}
                    \item We might only need distance to 100-th nearest neighbour (e.g. for distance based outlier detection), but need to find all the 100 nearest neighbours
                \end{itemize}
                \item Hard to parallelalize
                \item Combinatorial solutions aren't general
                \begin{itemize}
                    \item Hard/time-consuming to design new fast combinatorial method for new queries, or automate the process of designing algorithms
                    \item No combinatorial method can handle \textit{all} queries fast
                \end{itemize}
            \end{itemize}
            \item Learning-based methods
            \begin{itemize}
                \item Have been successfully applied to some database/combinatorial problems
                \item But no general neural network-based framework for learning
            \end{itemize}
        \end{itemize}


    \item \textbf{Neural Databases}
    \begin{itemize}
        \item Overview
        \begin{itemize}
            \item Database queries are functions
            \item Learn from sample queries and their answer
            \item Answer queries without data access
        \end{itemize}
        \item General method for answering any query approximately
        \item Takes advantage of data/query distribution
        \item Can be applied to any query
        \begin{itemize}
            \item The framework is general, but we show that it can be applied to queries with low-dimensional outputs
            \item higher-dimensional output needs more training samples to avoid over-fitting so are harder to learn
        \end{itemize}
        \item Scales easily with more computational power
        \item Differentiable database operations (possible applications in ML)
    \end{itemize}
    \item Neural Database vs. ML for combinatorial optimization
    \begin{itemize}
        \item Answers different queries on a particular database, compared with answering different instances of a problem type
    \end{itemize}
    \item Neural Database vs. existing ML use-cases for DB problems
    \begin{itemize}
        \item Ad-hoc ML use-cases, no general framework applicable to all problems
        \item Indexing \cite{kraska2018case} and aggregate queries \cite{ma2019dbest} are special cases
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item View of database queries as functions that can be learned
        \item Propose first general framework to answer queries efficiently using neural networks
        \item Design a model based on the framework
        \item Show how it can be applied to nearest neighbour/distance to nearest neighbour/range aggregate queries
        \item Experimentally show it does better than existing methods
    \end{itemize}
\end{itemize}

\fi

==> NeuroDB-ICDE (tech)/Architecture.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{overview_svg-tex.pdf}
    \vspace{-0.5cm}
    \caption{NeuroDB Framework}
    \label{fig:ndb}
\end{figure*}
\section{NeuroDB}\label{sec:NeuroDB}
To solve Problem \ref{prob:RAQ}, we design and train a function approximator in Sec.~\ref{sec:arch}. We show how it can answer queries in Sec.~\ref{sec:answering_queries} and analyze its performance in Sec.~\ref{sec:analysis}.

%In this paper, as motivated in Sec.~\ref{sec:intro:neurodb_RAQ}, we consider the class of function approximators to be neural networks. The parameter set $\Theta$ in Problem~\ref{prob:RAQ} can be defined as the class of all possible neural networks, in which case the problem becomes a neural architecture search problem \cite{zoph2016neural}. Given that neural architecture search and optimizing neural networks are still an active area of research, answering the above problem is difficult and brings together the research on approximation theory \cite{christensen2004approximation}, neural architecture search \cite{zoph2016neural} and databases. In this paper, we set $\Theta$ to a specific neural network architecture (to be specified in Sec. \ref{sec:arch}) that satisfies the storage and evaluation time requirement. Consequently, Problem \ref{prob:RAQ} becomes the problem of optimizing neural networks' parameters to answer a particular query function. We do this with a typical supervised learning approach. We discuss the specifics of our design in Sec.~\ref{sec:arch}, how the model is used to answer the queries in Sec.~\ref{sec:answering_queries}, extensions to general RAQS in Sec.~\ref{sec:raq_extension} and provide an analysis of the performance in Sec.~\ref{sec:analysis}.



\subsection{Model Architecture and Training}\label{sec:arch}
\subsubsection{Challenges}\label{sec:arch:challanges} Using neural networks to answer RAQs comes with its own challenges. We first discuss these challenges that motivate our design choices. 
%Multiple issues need to be addressed in designing a neural network for our purposes. 

\noindent(1) \textbf{Query time/accuracy trade-offs}. To improve the accuracy of a neural network, we need to increase the number of its parameters. Meanwhile, a forward pass of a neural network takes time linear in the number of its parameters (assuming no parallelization). A design is needed that can limit the increase in query time while improving accuracy. We avoid parallelization for fair comparison with existing methods, but its implications are discussed in Appendix~\ref{appx:parallel}.

%Thus, we need a systematic way to increase the capacity of the model to achieve the desired accuracy. 

%Another issue is designing a neural network with low query time when higher accuracy is desired (or when $n$ increases). 


\noindent(2) \textbf{Dependence on $n$}. The query function $f_D$ is dependant on the dataset $D$ and the complexity of approximating $f_D$ depends on the dataset and its size $n$. $f_D$ is a piece-wise constant function and increasing $n$ can increase the number of pieces. Intuitively, this is because the answer to a query changes only when the set of matching points to the range predicate changes. Thus, points of discontinuity can happen whenever a data point is on the boundary of the range predicate, as in those scenarios changing the range predicate by any non-zero amount can change the value of the query function by a fixed amount. This also implies that the number of discontinuities is larger when there are more points in a database. 
%Furthermore, at any point where the function is continuous, changing the range predicate by some small amount does not change the answer at all. 
%This can be seen in Fig. \ref{fig:visit_query_function_sampled}, where dropping the number of data points by a factor of 10 reduces the number of pieces that compose the function (also compare Fig.~\ref{fig:visit_query_function_sampled} and Fig.~\ref{fig:visit_query_function}). 
%As such, it is unlikely that the same neural network architecture is able to answer the query for different values of $n$ with the same accuracy. % and more parameters may be needed to approximate the more complicated function. 
Thus, our proposed architecture should be able to take data size into account. Fig.~\ref{fig:visit_query_function} (right) shows the piece-wise constant nature of the query function in our running example.

\noindent(3) \textbf{Training time}. Since number of parameters needs to increase with accuracy and data size, training could become harder and take more time and space. Although training time is a preprocessing step and does not affect query time, training of the network should be feasible with existing GPUs.

%\noindent(1) \textbf{Dependence on $n$}. The query function $f_D$ is a function dependant on the database $D$. Thus, the complexity in approximating $f_D$ depends on the dataset and its size $n$. Generally, as $n$ increases, the function to be approximated can become more \textit{complicated} and it is unlikely that the same neural network architecture is able to answer the query for different values of $n$ since more parameters may be needed to be able to approximate the more complicated function. ferent values of $d$, the query space may change. This will change the dimensionality of the input to the neural network, which necessitates changing its number of parameters (so that the first layer takes into account all the dimensions). 
\if 0
\begin{figure}
    \centering
    \begin{minipage}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{h_hst_0.01_pred_10_sp_692.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\columnwidth}
    \includegraphics[width=\textwidth]{h_hst_0.01_pred_10_sp_6925.png}
    \end{minipage}
    \caption{Average visit duration RAQ function on a sub-sampled database with 692 (left) and 6,925 (right) points.}
    \label{fig:visit_query_function_sampled}
\end{figure}



[0, 3): 3: 6
[3, 6): 6: 8
[6, 9): 9: 7


3, 6
6, 8
9, 7

[0, 1): 1, 2, 3: 5.6
[1, 2): 2, 3: 6.5
[2, 3): 3, 5: 3
[3, 5): 5, 6: 4
[5, 6): 6, 8: 6.5
[6, 8): 8, 9: 6
[8, 9): 9:  7

1, 4
2, 7
3, 6
5, 0
6, 8
8, 5
9, 7
\fi


%\noindent(2) \textbf{Query time}. Another issue is designing a neural network with low query time when higher accuracy is desired (or when $n$ increases). Assuming no parallelization, a forward pass of a neural network takes time linear in the number of its parameters. To improve accuracy, we need to increase the number of parameters of our model, which may in turn increase the query time. A design is needed that can limit the increase in query time. We avoid parallelization to provide a fair comparison with existing methods, however, potential implications of parallelization are discussed in Sec. \ref{sec:analysis}.

%s also observed in [XX], a single forward pass of a small neural network on a GPU with tensorflow [XX] takes a long time (exact?), due to the time it takes to transfer the data from GPU to main memory. Thus, we train the neural network on GPUs, but at query time perform our forward passes on a CPU. Furthermore, for fair comparison with other methods, we avoid parallelizing our forward pass ). 





\if 0
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/ndb.eps}
    \caption{NeuroDB Framework}
    \label{fig:ndb}
\end{figure}
\fi




\subsubsection{Architecture and Training} 
NeuroDB consists of multiple neural networks with identical structures. At a preprocessing step, we split the query space into a number of partitions and learn a different neural network to answer the queries for each partition. At query time, to answer a new query, we find which neural network is responsible for it and then perform a forward pass of that neural network. The answer to the query is the output of the neural network.

Fig.~\ref{fig:ndb} shows this framework for our average visit distribution RAQ example. Here, based on the formulation in Sec.~\ref{sec:def}, the query space is the possible bottom-left co-ordinates of the query rectangle. Fig.~\ref{fig:ndb} shows that in a preprocessing step, the query space is partitioned into 4 partitions. Then, for the $i$-th partition, a model, $\hat{f}_D^i(.; \theta)$, is learned that mimics the query function $f_D(.)$ for that part of the query space. Subsequently, the partitions are indexed. Finally, given a new query, $q_n$, the index is traversed to find which partition it belongs to. A forward pass of the corresponding neural network is performed and the output is returned as the answer, in this case  $\hat{f}_D^2(q_n; \theta)$.

%and a fixed architecture is used for all the neural networks. Thus, the total number of parameters used is equal to the number of parameters per architecture times $N_p$. 

%Fig. \ref{fig:ndb} shows this architecture. Fig. \ref{fig:ndb} (left) shows that the query space is partitioned into smaller partitions and Fig. \ref{fig:ndb} (right) shows how a tree structure is built with a neural network at each leaf node. A query traverses the tree until it reaches a leaf node, and then a forward pass of the neural network is performed.

%, and to increases or decrease the number of parameters we adjust the height of the index (which increases the number of neural networks used).

%an \textit{index} where each \textit{leaf} contains a neural network. The index decides which neural network is responsible for which query, and the corresponding neural network is used to answer the query. 

%The index partitions the \textit{query space} into multiple partitions, and a separate neural network is learned for each partition. 
Before explaining the specifics of our design, we discuss how this architecture addresses the challenges of Sec. \ref{sec:arch:challanges}. (1) Query time depends on the time it takes to find the partition the query belongs to, $t_p$, and the time of a forward pass for the neural networks, $t_n$. Using our architecture, increasing number of partitions increases $t_p$ but not $t_n$. Given that indexing can be used to search the partitions, $t_p$ is generally very small and increasing it has negligible impact on query time. As a results, we can increase number of parameters and model capacity at a low cost for query time. (2) Number of partitions can be used to increase the size of the architecture with data size and can be set as a function of $n$. (3) Training can be done independently for each neural network used. The benefits of this is twofold. First, neural networks can be trained in parallel and even on different devices, which speeds up training. Second, training requires less memory because all the networks do not need to be loaded at once. Thus, we can train only as many networks as there is memory for, as opposed to having to train all the network at once which requires larger memory. 


To summarize, this approach requires a method for partitioning the space and indexing them, as well as designing a neural network and training it for each partition. Our method uses a kd-tree to partition the space and index them,  and these steps are performed together. Thus, we first discuss those two steps and then discuss training of the neural networks. 


\noindent\textbf{Partitioning}. For this method to be successful, a good partitioning method needs to be chosen. Although it may be possible to learn the partitioning, our experiments showed that learning the partitioning is difficult and computationally intensive in practice. %For instance, consider the method of \cite{kraska2018case} that learns an index by optimizing a loss over the entire index structure. Adapted to our setting, that means that all the neural networks need to be optimized jointly, which significantly increases training time, and requires large memory for training (our technical report \cite{techreport} contains the methodology and results for an attempt to learn a partitioning). 
Instead, we take a different approach towards partitioning the space. Recall that our objective is to minimize $E_{q\sim \mathcal{Q}}[\Delta_{f_D}(q, \hat{f}_D(q;\theta)]$ which is $\sum_i p(q\in P_i)E_{q\sim \mathcal{Q}_i}[\Delta_{f_D}(q, \hat{f}_D(q;\theta)]$, where $P_i$ is the $i$-th partition and $\mathcal{Q}_i$ is the distribution of queries in partition $P_i$ (i.e., if $g_\mathcal{Q}(q)$ is p.d.f. of $\mathcal{Q}$, p.d.f. of $\mathcal{Q}_i$ is $\frac{g_\mathcal{Q}(q)}{p(q\in P_i)}$ if $q\in P_i$ and 0 otherwise). Thus, for each partition, its contribution to our objective is dependant on probability of it being queried as well as the average approximation error, where the former depends on the query distribution while the latter depends on the complexity of the function being approximated. Hence, we should select partitions such that high probability areas are approximated accurately, while the error for low probability partitions can be higher. We use the general observation that reducing the size of the space approximated by a neural network allows for better approximations in the smaller space. We choose partitions that are smaller where the queries are more frequent and larger where they are less frequent. This can be done by partitioning the space such that all partitions are equally probable. 

To this end, we build a kd-tree on our sampled query set, $Q$. Note that the split points in the kd-tree can be considered as estimates of the median of the distribution $\mathcal{Q}$ (conditioned on the current path from the root) along one of its dimensions obtained from the samples in $Q$. We build the kd-tree by specifying a maximum height, $h$, and splitting every node until all leaf nodes have height $h$, which creates $2^h$ partitions. Splitting of a node $N$ is done based on median of one of the dimensions of the subset, $N.Q$, of the queries, $Q$, that fall in $N$. Thus, a leaf node will have at least $\lfloor\frac{|Q|}{2^{h-1}}\rfloor$ queries. The complete procedure is shown in Alg.~\ref{alg:get_index}. To build an index with height $h$ rooted at a node, $N_{root}$ (note that $N_{root}.Q=Q$), we call $get\_index(N_{root}, h, 0)$ defined in Alg.~\ref{alg:get_index}. %The procedure builds a kd-tree, where each node, $N$, splits the space into two, based on the median of one of the dimensions $N.Q$. As the kd-tree is being built, the query set $Q$ is pushed down the tree, . % and one way to choose $h$ is by making sure the number of query samples per partition is not too small for training. 

%The split points in the kd-tree can be considered as estimates of the median of the distribution $\mathcal{Q}$ (conditioned on the current path from the root) along one of its dimensions, obtained from the samples in $Q$. This may seem unconventional as kd-trees are generally built on the data points and not the queries, but we emphasize that the goal of building a kd-tree is to partition the query space.  However, we note that the number of data points that fall into a partition do impact the difficulty of approximating the query function, and incorporating them in the partitioning can be an interesting future direction.


\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE A kd-tree node $N$, tree height $h$ and dimension, $i$ to split the node, $N$ on 
\ENSURE A kd-tree with height $h$ rooted at $N$
\IF{$h=0$} 
    \STATE $N.model \leftarrow train\_model(N.Q, f_D(N.Q))$\label{alg:get_index:train}
    \RETURN 
\ENDIF
\STATE $N.val\leftarrow$ median of $N.Q$ along $i$-th dimension
\STATE $N.dim\leftarrow i$
\STATE $Q_{left}=\{q|q\in N.Q, q[N.dim]\leq N.val\}$
\STATE $Q_{right}=\{q|q\in N.Q, q[N.dim]>N.val\}$
\FOR{$x\in \{left, right\}$}
    %\STATE $Q_l, Q_r\leftarrow$ Split $Q$ into two sets based on $m$
    \STATE $N_x$ $\leftarrow$ new node
    \STATE $N_x.Q\leftarrow Q_x$
    \STATE $N.x\leftarrow N_x$\TRICOMMENT{Adding $N_x$ as left or right child of $N$}
    \STATE $get\_index(N_x, h-1, (N.dim+1)\mod d_{pred})$
\ENDFOR
\end{algorithmic}
\caption{$get\_index(N, h, i)$}\label{alg:get_index}
\end{algorithm}



\noindent\textbf{Training}. We train an independent model for each of the $2^h$ leaf nodes. For a leaf node, $N$, this happens in Line \ref{alg:get_index:train} of Alg.~\ref{alg:get_index}, where the function $train\_model(N.Q, f_D(N.Q))$ returns a trained model on the training data $N.Q$ and $f_D(N.Q)$. $N.Q$ are query samples that fall within the part of the query space that node $N$ is responsible for. $f_D(N.Q)$ is used as the training label for queries in $N.Q$. Note that the answers can be collected through any known algorithm, where a typical algorithm iterates over the points in the database, pruned by an index, and for a candidate data point checks whether it matches the RAQ predicate or not.
%To keep our discussion generic to any RAQ, we avoid specifying what algorithm should be used to collect the answers to the queries. In the absence of any efficient algorithm, finding the set of matching point to the predicates can be done in time $O(|D|\times|Q|)$, where, for each query point, we iterate through each data point and check whether it matches the RAQ predicate or not, assuming that checking whether a point $p\in D$ matches a predicate parameterized by $q\in Q$ can be done in constant time (in most cases, this processes can be improved significantly by indexing the data points). 
We emphasize that this is a pre-processing step. That is, this sample collection step is only performed once and is only used to train our model. Furthermore, the process is embarrassingly parallelizable across training queries, if preprocessing time is a concern. %We experimentally show in Sec. \ref{sec:exp} that after training the model, NeuroDB can answer the queries orders of magnitude faster than the algorithm it used for this pre-procesing step.

%To train a model, we need access to samples of the form $(q, f_D(q))$, where $f_D(q)$ is the correct answer for the query $q$. Given that we have a set $Q$ of sampled queries, we only need access to some algorithm that can be used to answer $q$, for each $q\in Q$. We note that this implies that we already know of an algorithm that can solve the query. However, we emphasize that this is a pre-processing step. That is, this sample collection step is only performed once and is only used to train our model. We experimentally show in Sec. \ref{sec:exp} that after training the model, NeuroDB can answer the queries orders of magnitude faster than the algorithm it used to learn from. This is particularly useful because polynomial time solutions exist for many database queries, and thus sample collection can be easily performed. Subsequently, a NeuroDB can be trained to answer the queries efficiently. Besides faster query performance in general, this is specifically beneficial when the queries need to be answered on resource constrained devices (e.g., the model can be trained on a more powerful machine and deployed on IoT edge devices). 

The process of training is similar to a typical supervised training of a neural network with stochastic gradient descent (SGD). We use Adam optimizer \cite{kingma2014adam} for training and use a squared error loss function, that is, for the $i$-th partition corresponding to the leaf node $N$, the minimization objective is $\frac{1}{|N.Q|}\sum_{q\in N.Q}(f_D(q)-\hat{f}_D^i(q;\theta))^2$. %Finally, although we mentioned that we have access to a set $Q$ sampled from $\mathcal{Q}$, an interesting question for the future work is whether we can utilized samples not from $\mathcal{Q}$ to learn better models. 
\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE kd-tree root node $N$ and query $q$
\ENSURE Answer to $q$
\WHILE{$N$ is not leaf}
    \IF{$q[N.dim] \leq N.val$}
        \STATE $N \leftarrow N.left$
    \ELSE
        \STATE $N \leftarrow N.right$
    \ENDIF
\ENDWHILE
\RETURN $N.model.forward\_pass(q)$
\end{algorithmic}
\caption{$get\_answer(N, q)$}\label{alg:get_answer}
\end{algorithm}

\noindent\textbf{Neural Network Architecture}. We use a fully connected neural network for each of the partitions. The architecture is the same for all the partitions and consists of $n_l$ layers, where the input layer has dimensionality $d_{pred}$, the first layer consists of $l_{first}$ units, the next layers have $l_{rest}$ units and the last layer has 1 unit. We use relu activation all the layers (except the output layer). %Observe that, seen as a function of input dimensionality, the network size is $O(d_{pred})$, where the number of parameters for the network architecture are considered to be constant.
Note that $n_l$, $l_{first}$ and $l_{rest}$ are hyper-parameters of our model. Although approaches in neural architecture \cite{zoph2016neural} search can be applied to find them, they are generally computationally expensive. In this paper, we use a simple heuristic. We select one of the partitions, and do a grid search on the hyper-parameters. Since our neural network architecture for each partition is small, this grid search can be done in a practical time frame. The grid search finds the hyper-parameters so that NeuroDB satisfies the space and time constraints in Problem~\ref{prob:RAQ} while maximizing its accuracy. 

%Given that neural architecture search and optimizing neural networks are still an active area of research, answering the above problem is difficult and brings together the research on approximation theory \cite{christensen2004approximation}, neural architecture search \cite{zoph2016neural} and databases. In this paper, we set $\Theta$ to a specific neural network architecture (to be specified in Sec. \ref{sec:arch}) that satisfies the storage and evaluation time requirement. 

%Although approaches in neural architecture search can be applied to find them, they are generally computationally expensive. . Note that there is a time/space/accuracy trade-off when selecting the model architecture. Increasing the size of the the model increases the query time and space, but can improve accuracy.
%Hence, there are two ways to increase the number of parameters in an NeuroDB: increasing $h$ or increasing the number of parameters of each model. Increasing $h$ is generally preferred because it has very little impact on query time (increasing $h$ by one double the number of parameters but only add one extra comparisons). On the other hand, increasing the number of parameters of a model by creating deeper models allows for a more expressive network which allows for better accuracy \cite{telgarsky2016benefits}. 
%An interesting problem we experimentally study in Sec.~\ref{sec:exp} is choosing the smallest architecture possible that allows for a good enough accuracy.

\subsection{Answering Queries}\label{sec:answering_queries}
Answering queries using our NeuroDB framework is simple. The pseudocode is shown in Alg.~\ref{alg:get_answer}. For a query, $q$, first, the kd-tree is traversed to find the leaf node that the query $q$ falls into. The answer to the query is a forward pass of the neural network corresponding to the leaf node.

\vspace{-0.2cm}
\subsection{Analysis}\label{sec:analysis}
Given a value of $h$, there are $2^h$ partitions and each contains a neural network. We let $h=\log \frac{n}{c}$ for some user parameter $c$ denoting the \textit{capacity} of a neural network, so that the number of partitions, $N_p$, is $\frac{n}{c}$. That is, we increase the number of partitions linearly in $n$. %To define the capacity of a neural network, assume data points are sampled from a distribution $\mathcal{D}$, and that $S_c$ is a set of $c$ points sampled from $\mathcal{D}$. We define the capacity of a neural network $\hat{f}_D(q;\theta)$ as the largest number of points, $c$, such that $E_{S_c\sim D}[\Delta_{f_D}(q, \hat{f}_D(q;\theta))]\leq \epsilon$ for some error requirement $\epsilon$, when the neural network is trained on a training set $Q$. 
Intuitively, the capacity of a neural network denotes how \textit{complex} of a function it can approximate well, which depends on the number of neural network parameters, number of points in the database (as well as their distribution) and number of training samples available. We leave a theoretical study of the capacity of a neural network to the future work, but briefly mention that recent work on \textit{memorization capacity} of a neural network \cite{yun2019small} can be seen as a first step in this direction. We revisit the topic of what value of $h$ should be chosen empirically in our experiments. Regarding time and space complexity, for a fixed neural network architecture but variable data size and dimensionality, there will be $O(d_{pred}n)$ number of parameters, which means the space complexity is $O(d_{pred}n)$. Furthermore, at query time, the kd-tree needs to be traversed which takes $O(\log n)$, and a forward pass of the neural network takes $O(d_{pred})$. Thus, time complexity of the algorithm is $O(\log n +d_{pred})$. 

We acknowledge that, similar to recent learning-based approaches \cite{hilprecht2019deepdb, ma2019dbest} we do not provide an analytical formulation of the accuracy of NeuroDB. Nevertheless, we experimentally show that this architecture can provide good accuracy in practice. In our experiments, we discuss how model accuracy depends on number of training samples available, number of partitions and the size of each neural network.  

Regarding training time, given a network architecture, and assuming $T$ iterations of stochastic gradient descent, training time can be quantified as $O(d_{pred}nT)$, where each iteration for each network takes $O(d_{pred})$ and there are $O(n)$ networks.

  



%Roughly speaking, given a fixed model, the parameter $c$ can be used to control for accuracy. That is, reducing $c$ increases the number of partitions and the number of neural networks used, which improves accuracy. This logarithmically impacts runtime 


  
%\noindent\textbf{Comparison with Voronoi Diagram}. Finally, we contrast NeuroDB with Voronoi diagrams to provide more insights into our approach. For the purpose of this section assume the query in question is a nearest neighbour query. A Vornoi diagram partitions the query space, and answers queries based on which partition they fall into. The first observation is that, for the nearest neighbour query, a Voronoi diagram partitions the space such that the answer to the query is a \textit{constant function} in each partition. As a result, there are many partitions, but approximating each partition is very easy and can be done with just a constant function and with zero approximation error. However, exponentially many partitions need to be created in high dimensions \cite{arya1998optimal} which means storing and searching the partitions becomes difficult. Overall, we can see the same framework of partitioning the query space and then approximating each partition. In case of Voronoi diagram, the partitioning is the computationally challenging task while the approximation task is easy. NeuroDB can be seen as a method that transfers the cost of the partitioning task to the approximation task. Because the approximation method, i.e., neural networks, can perform well on high dimensional spaces, NeuroDB can avoid exponential blow-up in its size or query time. 


%Two methods can be used depending on whether we have access to the query distribution $\mathcal{Q}$ (and thus we can generate as many samples as required) or only a finite sampled query set $Q$. If only $Q$ is available, 



%How many paritions, relationship between no. partitions and size of NN, query time, training time

%Capacity of NN, B+-tree, voronoi


%First explain kd-tree, then mention why not a learned index

%Our framework is shown in Fig. \ref{fig:arch}. The architecture consists of two parts \textit{base} and \textit{index}. To limit the dependence of query time on $n$, we propose an architecture in which only a small part of the network needs to be executed, similar to [X, X].  To do so, we propose an \textit{index} architecture (in fac) The above mentioned challenges  , We need to specify a model architecture dependant on $n$ and $d$. Due to the nature of the problem, There are several difficulties that arise in selecting a model architecture. 



%The training and testing set contains pairs of the form $(q, f_D(q))$ where $q\sim \mathcal{Q}$. $f_D(q)$ is used as the label. Generally speaking, since the function $f_D(q)$ is available and in many cases can be evaluated in polynomial time, we may have access to an \textit{infinite} number of samples. However, we may not have access to $\mathcal{Q}$ and so may not be able to generate infinitely many samples based on $\mathcal{Q}$. 

\if 0
\begin{itemize}
    \item Select a neural network architecture
    \item Collect training and testing samples
    \begin{itemize}
        \item Need some way of answering queries to be able to collect samples
    \end{itemize}
    \item Train the network, estimate the expected error with validation set
\end{itemize}
\subsection{Model Architecture}
\begin{itemize}
\item Dependence of model to no. training samples
\item It is important to note that the query function $f_D$ depends on the query type, as well as the database $D$. This means that the function to be approximated is dependent on both data size and dimensionality. 

    \item General index+storage design
    \item Discuss the kd-tree
    \begin{itemize}
        \item Why we need it
        \item GPU vs. CPU
        \item How its built
    \end{itemize}
    \item Impact of model size on query time/storage size/accuracy
    \item Impact of data size, query dim., training size and how it relates to model parameters and training time
    \item Parallelism
\end{itemize}
\fi

==> NeuroDB-ICDE (tech)/Conclusion.tex <==
\vspace{-0.3cm}
\section{Conclusion}\label{sec:conclusion}
%We discussed how queries can be considered as functions that can be approximated, and formulated the general problem of learning models that can answer different databse queries. 
We introduced NeuroDB, a neural network framework for efficiently answering RAQs and distance to nearest neighbour queries, with orders of magnitude improvement in query time over the state-of-the-art algorithms.
%We discussed the challenges of designing such a framework such that it performs well in practice and can be trained easily, and how NeuroDB overcomes these challanges. 
We further showed that the same framework and neural network architecture can be used to answer both query types, showing the potential for utilizing a single framework to answer different query types and minimizing human time spent on designing algorithms for different query types. %We also showed that as a byproduct NeuroDB provides a differentiable query operator which may find applications in machine learning and feature learning. We further demonstrated that NeuroDB learns generalizable pattern between query input and output which may prove useful when there is missing data. 
To improve NeuroDB, future work can focus on parallelism, better partitioning methods and understanding theoretical guarantees of the accuracy of the method. Model pruning methods \cite{blalock2020state} that remove some of the \textit{unimportant} model weights can also be considered to reduce model size and evaluation time for faster performance, at the cost of accuracy. Additionally, studying NeuroDB for dynamic data and changing query distribution can be an interesting future direction. A straightforward approach can be to frequently test NeuroDB on a (potentially changing) test set, and re-train the neural networks whose accuracy fall below a certain threshold, but it may be possible to update the neural networks more cleverly. The general problem of updating a neural network is studied in the machine learning literature and is an active area of research \cite{quionero2009dataset, long2017deep, wang2019transferable, liu2019transferable}. However, interesting problems arise in the case of NeuroDB, since insertion of a new data point changes the query function in a specific and query dependent way. % (not all the neural networks in NeuroDB may need to be re-trained, as only some of the partitions may be affected by new data points).

%\noindent\textbf{Applicability to Other Query Types}. Although our framework is query-type agnostic and it can efficiently answer the database queries we discussed, its applicability to other query functions can be limited by (1) availability of enough samples, (2) complexity of the required model and (3) difficulty in obtaining a corresponding algorithm for training. The more complex the query function is, the more training samples are needed to train the model, using a corresponding algorithm to the query instances for training is more difficult, and a larger model is needed (the larger the model, the slower will be the query time). This is the reason we have made a distinction between \textit{distance to} nearest neighbour query and the nearest neighbour query. Although they both have the same combinatorial algorithms to answer them (we need to find the nearest neighbour to know the distance to the nearest neighbour), approximating one with a neural network is easier than the other. We believe that issues (1) and (2) will be addressed in the future. Special hardware for performing matrix multiplication are expected to become more powerful and prevalent \cite{kraska2018case}, and methods to generate more samples from the same distribution as some observed samples are already being studied in the literature \cite{thirumuruganathan2019approximate}. Regarding (3), we note that our method is useful when some polynomial algorithm is known for the query, which is used to obtain the correct answer for queries during training (we emphasize that this algorithm is only used to train our model in a preprocessing step, and is not used at test time). In practice, if the above issues exist in a system, an existing method can first be used to answer users' queries, while every answered query is also used to train NeuroDB. After NeuroDB reaches a certain accuracy threshold, it can replace the method it learned from for better efficiency. 


%\noindent\textbf{Potential for Machine Learning}. NeuroDB provides a differentiable database operation which may find potential applications in areas of machine learning such as contrastive learning \cite{chen2020simple}. Generally speaking, contrastive learning is a method used for feature learning where similar points are forced to be mapped to embeddings that are close in the feature space. Having a differentiable method that allows for measuring distance to nearest neighbours can allow for better enforcement of this requirement.  

%\noindent\textbf{The Learned Database Problem}. In the context of the learned database problem defined earlier, we have shown that even restricting our search space to a specific neural network architecture (and even without guaranteeing an optimal solution), we can learn a function approximator that can outperform existing methods for different query types. An open problem is whether expanding the algorithm space, e.g. to the set of all possible neural networks can improve the performance or not. Moreover, it can be interesting to analytically study the problem, to understand what class of function approximators should be used to learn to perform a query.




==> NeuroDB-ICDE (tech)/Definitions.tex <==
%\section{Problem of Learning Range Aggregate Queries}


\section{Problem Definition}\label{sec:def}
\noindent\textbf{Range Aggregate Queries}. Consider a dataset (or table) $D$ with $n$ records and with $d$ attributes, $X_1$, ..., $X_d$. For ease of discussion, we start by considering range aggregate queries that can be represented by the following SQL query. Such a query captures many real-world RAQs \cite{ma2019dbest}. We discuss the extension of our solution to more general RAQs in Sec.~\ref{sec:raq_extension}. 

\begin{tabular}{c}
\centering
\hspace{-0.7cm}
\begin{lstlisting}
SELECT $AGG$($X_m$) FROM $D$
WHERE ($x_1^l \leq X_1  < x_1^u $) AND ... AND ($x_d^l \leq X_d  < x_d^u $)
\end{lstlisting}
\end{tabular}

In the above SQL statement, for any $i$, $x_i^l$ and $x_i^u$ are \textit{query variables}, and they, respectively, define lower and upper bounds on the range of the attributes. For any $i$, $x_i^l$ and $x_i^u$ can be $-\infty$ and $\infty$ respectively, in which case there are no restriction on the values of $X_i$ in the query. We say that an attribute is \textit{not active} in the query in that case, and is \textit{activate} otherwise. Furthermore, $AGG$ is a user defined \textit{aggregation function} (typical examples include $SUM$, $AVG$ and $COUNT$), and $X_m$, for $1\leq m\leq d$, is the \textit{measure attribute}. For ease of discussion, we assume the measure attribute and the aggregation function are fixed, that is, we are only interested in answering RAQs with measure attribute $X_m$ and aggregation function $AGG$. We relax this assumption when discussing general RAQs in Sec.~\ref{sec:raq_extension}. Furthermore, let $q=(x_1^l, ..., x_d^l, x_1^u, ..., x_d^u)$ be a $d_{pred}$-dimensional vector for $d_{pred}=2\times d$. We call $q$ a \textit{query instance} and we assume query instances follows some distribution $\mathcal{Q}$. Thus, different query instances correspond to different range predicates for the measure attribute $X_m$ and aggregation function $AGG$.

We use a real-world database of location signals as our running example. The database, shown in Fig.~\ref{fig:visit_query_function} (left) contains latitude and longitude of GPS signals obtained from cell-phone devices and, for each location signal, the duration the user stayed in that location (more details about the dataset are provided in Sec. \ref{sec:exp}). The dataset is for downtown Houston, plotted on the map obtained from \url{maps.google.com}. Setting $X_1$, $X_2$ and $X_3$ to represent lat., lon. and visit duration attributes, respectively and $m=3$ and $AGG$ as $AVG$, the SQL statement above is the query of average visit duration for check-ins that fall in a rectangle with bottom left corner at $(x_1^l, x_2^l)$ and top right corner at $(x_1^u, x_2^u)$, and whose visit duration is between $x_3^u$ and $x_3^l$. The distribution $\mathcal{Q}$ decides which query instance are more common than others. $\mathcal{Q}$ may ensure $x_3^l=-\infty$ and $x_3^u=\infty$ with probability 1, since visit duration is typically not an active attribute, or, $(x_1^l, x_2^l)$ and $(x_1^u, x_2^u)$ may follow a distribution so that the range is more often around POIs in downtown rather than residential areas. 





 %Finally, note that the set $P$ can be written as $\{x|x \in \mathcal{D}, p(x, q)=1\})$, and that for a predicate variable $q$, predicate function $p$ and an aggregation function $AGG$, the answer to an RAQ can be written as $AGG(\{x|x \in D, p(x, q)=1\})$. In this paper, we focus on range predicates that can be represented by a query variable and a predicate function.

%. , but some examples follow. $q$ can be a lower bound on an attribute and $p(q, x) = x[0]>q[0]$. We can also have $p(q, x) = x[1]>x[0]\times q[0]+q[1]$, in which case $p(q, x)$ and $q$ define a half-space above a line specified by $q$. For a predicate variable $q$, predicate function $p$ and an aggregation function $AGG$, the answer to an RAQ can be written as $AGG(\{x|x \in D, p(x, q)=1\})$. In this paper, we focus on range predicates that can be represented by a query variable and a predicate function.

\noindent\textbf{Query Functions}. Such RAQs can be represented by a function of the query instance. %Let $q=(x_1^l, ..., x_d^l, x_1^u, ..., x_d^u)$ be a $2\times d$-dimensional vector. Then, 
Define the function $f_D(.)$ so that for a query $q$, $f_D(q)$ is the answer to the above SQL statement. We call $f_D(.)$ a \textit{query function}. A \textit{query instance} defines a particular query on a database, and a \textit{query function} is a function that maps a query instance to its answer. In our running example, the function $f_D(.)$ takes as input the ranges on three attributes (and thus, its input dimensionality is 6) and outputs a real number. In Fig. \ref{fig:visit_query_function} (right), we show this function for a subset of query instances. Specifically, it shows the query of average visit duration given a square of side length 0.00043 in geo-coordinates (which is about 50m) with bottom left corner at location $(x_1^l, x_2^l)$, which is achieved by setting $x_3^l=-\infty$, $x_3^u=\infty$, $x_1^u=x_1^l+0.00043$, $x_2^u=x_2^l+0.00043$.%, $m=3$ and $AGG=AVG$. 


%a query point $(c, r)$ corresponding to a rectangle range predicate where no data points are on the edges of the rectangle. Then, for a small enough $\epsilon$, the answer to query points, $(c', r)$, for $c'=c+\epsilon v$, where $v$ is a unit vector in any direction is the same as the answer to $(c, r)$ (because the set of matching points to predicate $(c', r)$ is the same as $(c, r)$). Furthermore, observe that inserting a new data point at $c+r+\frac{\epsilon}{2}$ increases the number of pieces, because it splits at least one of the pieces into two. Doing so results in the answers to query $(c+\frac{\epsilon}{2}, r)$ to be different from $(c, r)$. 



%Note that $f_D(q):I\rightarrow R$ where $I$ is the query space, i.e., the set of possible query instances for a particular predicate function. % and which includes all possible range predicates and aggregation functions. %Note that when referring to a query function the only variable is the choice of the range predicate. Thus, for simplicity, we often use $f_D(q)$ to refer to a query function, where $q$ denotes a range predicate. 


\noindent\textbf{Problem Statement}. Our goal in this paper is to learn a function approximator, $\hat{f}_D(.; \theta)$ that approximates the query function, $f_D(.)$, well. In the general problem setting, $\hat{f}_D(q; \theta)$ can be any algorithm, from a combinatorial methods that operates on the data to a neural network. For any such function approximator, let $\Sigma(\hat{f}_D)$ be its storage cost (e.g., for neural networks, number of parameters) and $\tau(\hat{f}_D)$ be its evaluation time or query time (e.g., for neural networks, the time it takes for a forward pass). Furthermore, let $\Delta(f(q), y)\geq 0$ be an error function that measures how bad a solution $y$ is when the actual answer is $f(q)$ for a query $q$, e.g., it can be defined as 0-1 loss or $\lVert f_D(q)-y\rVert$. The problem studied in this paper is learning to answer range aggregate queries with time and space constraints, formulated as follows.

\begin{problem}\label{prob:RAQ}
Given a query function $f_D(.)$, query distribution $\mathcal{Q}$, class of function approximators, $\Theta$, and time and space requirements $t$ and $s$, find 
$$\hspace{-0.1cm}\arg\min_{\theta\in \Theta} E_{q\sim \mathcal{Q}}[\Delta(f_D(q), \hat{f}_D(q;\theta))]  \text{ s.t. }\Sigma(\hat{f}_D)\leq s \text{, } \tau(\hat{f}_D)\leq t$$
\end{problem}

%The formulation of Problem \ref{prob:RAQ} allows for learning a function approximator that is able to mimic a query function well. 
In the problem formulation, $\Theta$ shows our modelling choice. 
%Denote by $acc_{\Theta}(s, t)$ the objective value of the optimal solution to the above problem. $acc_{\Theta}(s, t)$ determines the time/space/accuracy trade-off of a class of function approximators, $\Theta$. 
Furthermore, since we usually only have access to a set $Q$ of samples from $\mathcal{Q}$ but not the distribution, we aim at optimizing $\frac{1}{|Q|}\sum_{q\in Q}\Delta(f_D(q), \hat{f}_D(q;\theta)$ instead of $E_{q\sim \mathcal{Q}}[\Delta(f_D(q), \hat{f}_D(q;\theta)]$.


%\noindent\textbf{Example}.  



%Consider an RAQ on this dataset with the average aggregation function on visit duration, and with axis-parallel rectangles as its range predicate. The range predicate can be represented by query variables $c, r\in R^2$ and predicate function $P_f(c, r, x)$, where $c$ is a two dimensional vector representing the center of the rectangle in each dimension, and $r$ is a two dimensional vector representing the length of the edge of the rectangle in each dimension. $P_f(c, r, x)$ returns 1 if $c[i]-\frac{r[i]}{2} \leq x[i] \leq c[i]+\frac{r[i]}{2}$ for all $i\in \{0, 1\}$ and 0 otherwise. Let $f_D(c, r)$ be the above query function, which takes as an input the rectangle information (i.e., rectangle center and edge lengths) and outputs the average visit duration for that rectangle. Fig. \ref{fig:visit_query_function} (right) plots this query function when $r=0.00043$ in geo-coordinates (which is about 50m) as a function of only $c$. Problem \ref{prob:RAQ} is the problem of learning a function $\hat{f}_D(c, r; \theta)$ that approximate this function well. 

%Problem \ref{prob:RAQ} is the problem of learning a function $\hat{f}_D(c, r; \theta)$ that approximate this function well. 

\if 0
\begin{figure}
    \centering
    \includesvg[width=0.5\columnwidth]{constant_piece.svg}
    \caption{NeuroDB Framework}
    \label{fig:constant}
\end{figure}
\fi



%\noindent\textbf{Query Representation}. We consider range predicates that can be represented by a predicate function $p$ and a predicate variable $q$. We allow arbitrary predicate function $p$ and predicate variables $q$. In practice, they can be created based on the WHERE clause of SQL queries (e.g., for attributes X and Y, and the clause WHERE X between L\_1 and U or Y>L\_2 we define q=(L\_1, U,L\_2)). We briefly mention that multiple representations may be possible. For instance, in our running example, the axis-aligned rectangles can also be represented by the minimum and maximum values in each co-ordinate. In this paper, to keep our methodology applicable to any RAQ, we assume the representation is given, and leave the study of the impact of representation for specific queries to the future work. Our methods and discussion apply to any representation and our only assumption is that the range predicate can be represented with a predicate function and a predicate variable. This allows formulating the problem in Def. \ref{prob:RAQ}. 


\if 0




\begin{figure}
    \centering
    %\hspace*{-cm}
    %\begin{minipage}{0.3\textwidth}
    %\includegraphics[width=\textwidth]{KeyValueStore.eps}
    %\caption{Look-up in Key Value Stores}
    %\label{fig:keyval}
    %\end{minipage}
    %\hfill
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/NN_points.eps}
    %\caption{Nearest Neighbour Query}
    %\label{fig:NN}
    \end{minipage}
    \hfill
    \begin{minipage}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/range_count_points.eps}
    %\caption{Range Agg. Query}
    %\label{fig:DistNN}
    \end{minipage}
    \caption{Nearest neighbour, $f_D^1(q)$, distance to nearest neighbour, $f_D^2(q)$, (left) and range aggregate, $f_D^3(q)$, (right) query functions}
    \label{fig:query_functions}
\end{figure}



\subsection{Different Query Types}
\textbf{Key-value store lookups}
A key-value store is a set of key-value pairs $D=\{(k_i, v_i)\in K\times V, \forall i\}$, where $K$ is the domain of keys and $V$ is the domain of values. Generally, keys are the identifiers and values are the corresponding data stored for the identifier. We focus on look-up queries, where the queries are to return the corresponding value of given key, i.e. $f_D(q):D\rightarrow V$, $f_D(k_i)=v_i$, $\forall k_i\in D$ and $f_D(q)$ is undefined if $q\neq k_i$ for any $i$ (we focus on the case where queries are only on the keys that are already stored in the key-value store). 

Fig. \ref{fig:keyval} shows a key-value store with 5 keys. Observe that the function $f_D(q)$ returns $v_i$ for any $k_i$ as its input. $\hat{f}_D(q;\theta)$ is another function that exactly approximates $f_D(q)$ at $k_i, \forall i$. Thus, instead of evaluating $f_D(q)$, we can evaluate $\hat{f}_D(q;\theta)$ at all possible query points and obtain the same answer.

\noindent\textbf{Range-aggregate query}. Given a $d$-dimensional database $D=\{p_i\in \mathcal{R}^d\}$, an aggregation function $g:2^D\rightarrow \mathcal{R}$ and a query $q\in \mathcal{R}^{2\times d}$, where $q$ defines a hyper-rectangle in $d$ dimensions, define $f_D(q) = g(\{p \in q\cap D\})$ where $q\cap D$ is the set of points in $D$ that intersect the range defined by $q$. For instance, $g$ can be a count function, in which case $f_D(q)$ is the number of data points in $D$ that are in the query range $q$. If $g$ is a count function, we can observe that $f_D(q)$ is a step function, with points of discontinuity whenever boundaries of $q$ intersect data points in $D$. For the one dimensional database $D=\{1, 2, 3, 5, 6\}$, Fig. \ref{fig:query_functions} (right) shows the query function for count aggregation function, where queries are assumed to be of the form $(q, \infty)$ (i.e., the only input is beginning of the range).

\noindent\textbf{$k$-th nearest neighbour query}.
Given a $d$-dimensional database $D=\{p_i\in \mathcal{R}^d\}$, an integer $k$, and a query $q\in \mathcal{R}^d$, $k$-th nearest neighbour query is to find the points in $D$ whose distance to $q$ is the $k$-th smallest. For this query, $f_D(q):\mathcal{R}^d\rightarrow\mathcal{R}^{d}$. 

For the one same one-dimensional database mentioned above, Fig. \ref{fig:query_functions} (left) shows the $k$-th nearest neighbour query function for $k=1$ (Shown as $f_D^1(q)$ in the left figure). Observe that $f_D^1(q)$ is a step function, where the output of $f_D^1(q)$ is always a point in the database. $f_D^1(q)$ is constant over the query inputs whose nearest neighbour is the same, and points of discontinuity occur when the nearest neighbour changes (this happens at the mid-point between consecutive data points, shown by dashed lines in the figure). 

%Defining $\Delta_{f_D}(q, y)=|f_D(q)-y|$, we can study the accuracy of the approximation offered by $\hat{f}_D(q;\theta)$. The figure shows that $\Delta_{f_D}(q, \hat{f}_D(q;\theta))<\delta_0$, $\forall q\in \mathcal{R}$, so $E_{q\sim \mathcal{Q}}[\Delta_{f_D}(q, \hat{f}_D(q))]\leq \delta_0$. However,  $E_{q\sim \mathcal{Q}}[\Delta_{f_D}(q, \hat{f}_D(q))]$ may in fact be much lower than $\delta_0$, depending on the distribution $\mathcal{Q}$. 

\noindent\textbf{Distance to $k$-th nearest neighbour}. In addition to $k$-nearest neighbour query, we also consider the \textit{distance to the $k$-the nearest neighbour} query. That is, if $p$ is the $k$-the nearest neighbour of a query point $q$, then $f_D(q)=d(p,q)$ for some distance metric and $f_D:\mathcal{R}^d\rightarrow\mathcal{R}$. Distance to $k$-th nearest neighbour query is not traditionally studied separately from the nearest neighbour query, because combinatorial methods use a nearest neighbour algorithms to find the distance to the nearest neighbour. However, using neural networks we can directly calculate distance to the nearest neighbour without ever finding any of the nearest neighbours. Thus, we study the query separately. As noted previously, it is useful for various application such as active learning \cite{settles2009active, fujii1999selective} or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. Another application is for assessing probability of getting infected from a disease, such as COVID-19, based on user locations. Consider a database that contains the location of infected people and let the neareset neighbour queries be the location of healthy people. The goal is to find the probability of a healthy person getting infected based on how close they were to infected people, which is the distance to their nearest neighbour.  The red curve in Fig. \ref{fig:query_functions} shows this query for $d=1$ and $k=1$ (on the same database mentioned above). Observe that, in contrast to the nearest neighbour query, this query is continuous. Furthermore, its range is a single real number, as opposed to $\mathcal{R}^{d}$. %We will later see how these features impact learning.

\fi


\if 0
\begin{itemize}
    \item Define a database query as a real-valued function
    \item Define the optimization problem of approximating this real-valued function to minimize error given constraints on time and space
    \item Discuss that the function approximator should handle databases of different size, dimensionality and different query types, and that we use a neural network to do that
    \item Examples. Show how the problem definition applies to nearest neighbour and range aggregate queries 
\end{itemize}
\fi

==> NeuroDB-ICDE (tech)/Exp.tex <==


\if 0
\begin{figure}[t]
%    \begin{minipage}[t]{.24\textwidth}
%        \centering
%    	\includegraphics[width=\textwidth]{exp_figs/nn_dist_d_space.eps}
%    	\caption{Impact of $d$ on space}
%    	\label{fig:exp:dist_nn_d_space}
%    \end{minipage}
    \begin{minipage}[t]{.23\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{exp_figs/range_agg_n_time.eps}
    %\caption{Impact of $n$}
%    	\label{fig:exp:range_agg_n_time}
    \end{minipage}
    \begin{minipage}[t]{.23\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{exp_figs/range_agg_d_time.eps}
    	%\vspace{-0.7cm}
%    	\caption{Impact of $k$}
%    	\label{fig:exp:range_agg_d_time}
    \end{minipage}
    \caption{Results for range agg. query}
    \label{fig:exp:range_agg}
    %\begin{minipage}[t]{.24\textwidth}
    %    \centering
    %	\includegraphics[width=\textwidth]{exp_figs/range_agg_range_time.eps}
%    	\caption{Impact of $d$}
%    	\label{fig:exp:range_agg_range_time}
%    \end{minipage}
\end{figure}
\fi







%\vspace{-0.3cm}
\section{Empirical Study}\label{sec:exp}
In this section, we first empirically evaluate NeuroDB for RAQs in Sec.~\ref{sec:exp:rang_agg}. Then, we apply the same NeuroDB architecture to answer distance to nearest neighbour queries in Sec.~\ref{sec:exp:dist_NN}.
\if 0
\begin{itemize}
    \item What is the relationship between model hyperparameters and accuracy of NeuroDB? (Sec. \ref{sec:exp:hyperparam})
    \item Can NeuroDB provide better accuracy/time/space trade-offs than state-of-the-art and optimal combinatorial algorithms for the distance to nearest neighbour query? (Sec. \ref{sec:exp:dist_NN_res})
    \item Can the same NeuroDB architecture be used to answer range aggregate queries better than the state-of-the-art and query specific algorithms? (Sec. \ref{sec:exp:rang_agg})
    \item Can NeuroDB learn any useful patterns for the nearest neighbour query?  (Sec. \ref{sec:exp:NN})
\end{itemize}
\fi
%We summarize our findings in Sec. \ref{sec:exp:summary}.

\noindent\textbf{System Setup.} The experiments are performed on a machine running Ubuntu 18.04 LTS equipped with an Intel i9-9980XE CPU (3GHz), 128GB RAM and a GeForce TRX 2080 Ti NVIDIA GPU.

\noindent\textbf{Model Training and Evaluation}. For all the experiments, building and training of NeuroDB is performed in Python 3.7 and Tensorflow 2.1. Training of the model is done on GPU. The model is saved after training. For evaluation, a separate program written in C++ and running on CPU loads the saved model, and for each query performs a forward pass on the model. Thus, model evaluation is done with C++ and on CPU, without any parallelism for any of the algorithms. We refer to our algorithm as {NeuroDB}. Unless otherwise stated, we set the model depth to 5 layers, with the first layer consisting of 60 units and the rest with 30 units. The height of the kd-tree is set to 4. We found this architecture to provide both good accuracy and query time, but we also present results on impact of each of the hyperparamters. 



\subsection{Range Aggregate Query}\label{sec:exp:rang_agg}
\subsubsection{Setup}\hfill\\
\noindent\textbf{Dataset}. We use real, benchmark and synthetic datasets for evaluation. The data size and dimensionality for each dataset is shown in Table~\ref{tab:dataset_size}. For each dataset, we specify a measure attribute on which the aggregation function operates.

%eevery active attribute, we generate  range predicate consisting of conjunction of range clauses over  multiple columns in the database. Specifically, we consider predicates specified by the predicate function $P_f(q_l, q_u, x, C)$, for query variables $q_l$ and $q_u$, data point $x$ and list of database column names $C$, where $P_f(q_l, q_u, x, C)$ is equal to 1 if for all $c\in C$, $q_l[c]\leq x[c] < q_u[c]$ and 0 otherwise. Note that for such a formulation, $d_{pred}$ is $2\times|C|$, which is the dimensionality of the input to the neural networks. We refer to $|C|$ as the dimensionality of an RAQ. We note that NeuroDB is not limited to predicate functions of this form, but we use such predicates to allow for comparison with existing learning-based methods, e.g., \cite{ma2019dbest, hilprecht2019deepdb}, that do not support arbitrary predicate functions. Finally, unless otherwise stated, we use AVG aggregation function, but we also consider SUM and STD. The details of the datasets used are as follows.

\noindent\textit{PM2.5}. PM2.5 \cite{liang2015assessing} contains PM2.5 statistics for locations in Beijing. Similar to \cite{ma2019dbest}, we let PM2.5 to be the measure attribute. %As in \cite{ma2019dbest}, we considered Dew Point (DEWP), Pressure (PRES) or Temperature (TEMP) as attributes for the range predicate. Here, we only report the results on PRES, as the performance of all algorithms on all attributes where similar. Thus, the predicate function used is $P_f(q_l, q_u, x, \{\text{PRES}\})$.

\noindent\textit{TPC-DS}. We used TPC-DS \cite{nambiar2016the} with scale factors 1 and 10, respectively referred to as TPC1 and TPC10. Since we study range aggregate queries, we consider the numerical attributes in store\_sales table as our dataset. We use net\_profit as the measure attribute. %attribute and consider range predicates on quantity, wholesale\_cost and sales\_price attributes. Our experiments consider predicate functions $P_f(q_l, q_u, x, \{\text{quantity}\})$, $P_f(q_l, q_u, x, \{$quantity, wholesale\_cost$\})$, $P_f(q_l, q_u, x, \{$quantity, wholesale\_cost, sales\_price$\})$.

\noindent\textit{Synthetic datasets}. To study the impact of data dimensionality and distribution, we generated synthetic 5, 10 and 20 dimensional data from Gaussian mixture models (GMM) with 100 components whose mean and co-variance are selected uniformly at random, respectively referred to as G5, G10 and G20. GMMs are often used to model real data distributions \cite{reynolds2009gaussian}. We set one of the columns to be the measure attribute. %To generate the data, for a column $X$, which is in the range predicate, the above distribution is used to generate its content, and for a column $Y$, which is the aggregation column, the values are generated uniformly at random. The predicate functions used is $P_f(q_l, q_u, x, \{\text{X}\})$.

\noindent\textit{Veraset}. As was used in our running example, we use Veraset dataset, which contains anonymized location signals of cell-phones across the US collected by Veraset \cite{veraset}, a data-as-a-service company. Each location signal contains an anonymized id, timestamp and the latitude and longitude of the location. We performed stay point detection \cite{ye2009mining} on this dataset (to, e.g., remove location signals when a person is driving), and extracted location visits where a user spent at least 15 minutes and for each visit, also recorded its duration. 100,000 of the extracted location visits in downtown Houston were sampled to form the dataset used in our experiments, which contains three columns: latitude, longitude and visit duration. We let visit duration to be the measure attribute. %The query workload in this dataset is to find average visit duration for the predicate function $P_f(q_l, q_u, x, \{\text{latitude, longitude}\})$. We note that this shows another realistic application of our method, where data aggregators can use NeuroDB to release their data to the public to improve both query time and space efficiency, rather than releasing it in its raw format. 

%Unless otherwise stated, the results are reported on TPC1. For all datasets, 


\noindent\textbf{Query Distribution}. Our experiments consider query functions consisting of average, sum, standard deviation and median aggregation attributes together with two different predicate functions. First, similar to \cite{ma2019dbest}, our experiments show the performance on the predicate function defined by the WHERE clause in Sec.\ref{sec:def}. We consider up to 3 active attributes in the predicate function. To generate a query instance with $r$ active attributes, we first select, uniformly at random, $r$ activate attributes (from a total of $d$ possible attributes). Then, for the selected active attributes, we randomly generate a range. Unless otherwise stated, the range for each active attribute is uniformly distributed. This can be thought of as a more difficult scenario for {NeuroDB} as it requires approximating the query function equally well over all its domain, while also giving a relative advantage to other baselines, since they are unable to utilize the query distribution. Unless otherwise stated, for all dataset except Veraset, we report the results for one active attributes and use the average aggregation function. For Veraset, we report the results setting latitude and longitude as active attributes. Second, to show how NeuroDB can be applied to application specific RAQs, in Sec.\ref{exp:veraset}, we discuss answering the query of median visit duration given a \textit{general} rectangle on Veraset dataset. 

%We note that, unless otherwise stated, for PM2.5, TPC-DS and Synthetic datasets, the query workload consists of a range predicate on one attribute of the form $q[0]\leq X< q[1]$ for a query variable $q$ and attribute $X$ and for veraset, the range predicate i %We note that for a $d$-dimensional database, queries are $2\times d$-dimensional vectors, where for each dimension a minimum and maximum value is specified.%Unless otherwise specified, $n$ is set to 100,000 and $d$ is set to 2.


\noindent\textbf{Measurements}. In addition to query time and space used, we report the normalized absolute error for a query in the set of test queries, $T$, defined as $\frac{|f_D(q)-\hat{f}_D(q, \theta)|}{\frac{1}{|T|}\sum_{q\in T}|f_D(q)|}$. The error is normalized by average query result magnitude to allow for comparison over different data sizes when the results follow different scales. 

\begin{table}[t]
\hspace{-0.5cm}
\begin{minipage}{0.5\columnwidth}
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Dataset} & \textbf{\# Points} &\textbf{Dim}. \\\hline
        \begin{tabular}{@{}c@{}} G5, G10\\ G20 \end{tabular}
          & 100,000 & \begin{tabular}{@{}c@{}} 5, 10\\ 20 \end{tabular} \\\hline
        PM2.5 \cite{liang2015assessing} & 41,757 & 4 \\\hline
         %& 100,000 \\\hline
         %& 100,000 \\\hline
        %U & 100,000 \\\hline
        TPC1 \cite{nambiar2016the} & 2,653,123 & 13 \\\hline
        TPC10 \cite{nambiar2016the} & 26,532,166 & 13\\\hline
        Veraset (VS)  & 100,000 & 3
    \end{tabular}
    \caption{Datasets for range aggregate queries}
    \label{tab:dataset_size}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}{0.5\columnwidth}
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Dataset} & \textbf{\# Points}  & \textbf{Dim.} \\\hline
        \begin{tabular}{@{}c@{}}GloVe (GV)\\ \cite{pennington2014glove}  \end{tabular}  & 1,191,887 &
        \begin{tabular}{@{}c@{}}25, 50 \\ 100, 200  \end{tabular}
        \\\hline
        GIST \cite{gist} & 1,000,000 & 960 \\\hline
        KDD \cite{kdd} & 1,009,745 & 36 \\\hline
        IPUMS \cite{ipums} & 70,187  & 60
    \end{tabular}
    \caption{Datasets for distance to nearest neighbour query}
    \label{tab:nn_dataset_size}
\end{minipage}
\end{table}



\begin{figure*}[t]
    \begin{minipage}[t]{.49\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{RAQ_data.eps}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_acc_data.eps}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_time_data.eps}
    	    	\vspace{-0.65cm}
        \caption{RAQs on different datasets}
        \label{fig:exp:range_agg_data}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{RAQ_range.eps}
        \vspace{-0.65cm}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_agg_range_acc.eps}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_agg_range_time.eps}
        \caption{Impact of query range on RAQs}
        \label{fig:exp:range_agg_qrange}
    \end{minipage}
\end{figure*}
\begin{figure*}[t]
\vspace{-0.1cm}
    \begin{minipage}[t]{.49\textwidth}
        \centering
    	\includegraphics[width=1\textwidth]{RAQ_dim.eps}
    	\vspace{-0.65cm}
        \caption{Impact of number of active attributes on RAQ}
        \label{fig:exp:range_agg_dim}
    \end{minipage}  
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{RAQ_aggf.eps}    	
        \vspace{-0.65cm}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_acc_aggf.eps}
    	%\includegraphics[width=0.49\textwidth]{exp_figs/range_time_aggf.eps}
        \caption{Impact of agg. function on RAQs}
        \label{fig:exp:range_agg_aggf}
    \end{minipage}
\end{figure*}

\noindent\textbf{Baseline Algorithms}. We considered DBEst \cite{ma2019dbest} and DeepDB \cite{hilprecht2019deepdb} as the state-of-the-art model-based approximate query processing engines. Both algorithms learn models of the data and answer specific queries based on the models of the data. We use the open-source implementation of DBEst available at \cite{dbest_imp} and DeepDB at \cite{deepdb_imp}. In a preliminary experiment, we compared the performance of DBEst and DeepDB on TPC1, for queries with one active attribute and observe that DeepDB performs much better than DBEst. Furthermore, DBEst's implementation does not support multiple active attributes. Thus, we chose DeepDB as our model-based baseline. We use the default parameter setting for DeepDB. Furthermore, we use VerdictDB \cite{park2018verdictdb} as our sampling-based baseline, using its publicly available implementation \cite{verdict_imp}. We also implemented a sampling-based baseline designed specifically for range aggregate queries, referred to as TREE-AGG. In a pre-processing step and for a parameter $k$, TREE-AGG samples $k$ data points from the database uniformly. Then, for performance enhancement and easy pruning, it builds an R-tree index on the samples, which is well-suited for range predicates. At query time, by using the R-tree, finding data points matching the query is done efficiently, and most of the query time is spent on iterating over the points matching the predicate to compute the aggregate attribute required. For both TREE-AGG and VerdictDB, we set the number of samples so that the error is similar to that of DeepDB, as we assume the-state-of-the-art algorithm, DeepDB, answers the queries with an acceptable error rate.



%. To perform a query at random until the error falls bellow a specified error threshold. We use this algorithm due to its generality, as similar to {NeuroDB}, it can be applied to any range predicate and aggregation function. To improve the efficiency of the baseline, we first sample all the data-points, build an R-tree and then perform the range query on the R-tree (we consider the sampling and building the R-tree a pre-processing step, and exclude it from query time). This prunes the points that don't match the range predicate, and empowers the baseline to avoid performing direct comparison on those points.

\subsubsection{Results Across Datasets} Fig.~\ref{fig:exp:range_agg_data}  (a) shows the error on different datasets, where NeuroDB provides a lower error rate than the baselines. Fig.~\ref{fig:exp:range_agg_data} (b) shows that NeuroDB achieves this while providing multiple orders of magnitude improvement in query time. NeuroDB has a relatively constant query time. This is because, across all datasets, NeuroDB's architecture only differs in its input dimensionality, which only impacts number of parameters in the first layer of the model and thus changes model size by very little. Due to our use of small neural networks, we observe that model inference time for NeuroDB is very small and in the order of few microseconds, while the modeling choices of DeepDB leads to query time often multiple orders of magnitude larger. Furthermore, the results on G5 to G20 show the impact of data dimensionality on the performance of the algorithms. We observe that, for NeuroDB, the error increases as dimensionality increases, which is because the model needs to learn more information. The similar impact can be seen for DeepDB, manifesting itself in increased query time. Furthermore, the R-tree index of TREE-AGG often allows it to perform better than the other baselines, especially for lower dimensional data.  %how the number of data points affects query time for a fixed average error requirement, for the count aggregation function and $d=2$. Overall, the pattern is similar to that of distance to nearest neighbour query with {NeuroDB} providing orders of magnitude improvement over {ON-AGG}. {NeuroDB} changes very little as $n$ increases but there is a drastic impact on {ON-AGG}. We note that, given the same training size as distance to nearest neighbour, {NeuroDB} is able to support larger data sizes when answering range aggregate queries. This implies that, at least empirically speaking, range aggregate queries are easier to approximate compared with distance to the nearest neighbour (although we use a different error metric depending on the type of the query, which also has an impact). 


\subsubsection{Different Workloads on TPC1}
\hfill\\\noindent\textbf{Impact of Query Range}. We experimented with setting the query range to $x$ percent of the domain range, for $x\in\{1, 3, 5, 10\}$, presented in Fig.~\ref{fig:exp:range_agg_qrange}. We observe that error rate of NeuroDB increases for smaller query ranges since for smaller ranges NeuroDB needs to memorize where exactly each data point, rather then learning the overall distribution of data points which can be done for larger ranges. Nevertheless, NeuroDB provides better accuracy than the baselines for query ranges at least 3 percent, while performing queries orders of magnitude faster for all ranges. We note that if more accurate answers are needed for smaller ranges in an application, increasing the model size of NeuroDB can improve its accuracy at the expense of query time (as studied in Sec.~\ref{exp:veraset}).  
%Interestingly, performance of TREE-AGG improves with larger query range. This can be due to fewer samples being needed to answer queries with larger ranges since the ranges overlap more. Furthermore, accuracy of NeuroDB improves when the range increases, 


\noindent\textbf{Impact of no. of active attributes on Query Time}.  We vary the number of active attributes in the range predicate from one to three. The accuracy for all the algorithms drops when there are more active attributes, with NeuroDB outperforming the algorithms both in accuracy and query time. For NeuroDB, the drop in accuracy can be due to larger training size needed for higher dimensional data to achieve the same accuracy, while our training procedure is the same for all dimensions. %However, we note that performance of NeuroDB even on the 3-dimensional data is better than DBEst on one dimensions. We also observe that performance of DeepDB and TREE-AGG deteriorates with dimensionality. For TREE-AGG, this can be due to, first, difficulty in indexing, and second, that more samples are required to obtain similar accuracy. Although query time of NeuroDB remains similar, its accuracy worsens for larger dimensionality. 

\noindent\textbf{Impact of Aggregation Function}. Fig.~\ref{fig:exp:range_agg_aggf} shows how different aggregation functions impact performance of the algorithms. Overall, NeuroDB is able to outperform the algorithms for all aggregation functions. VerdictDB  and DeepDB implementation did not contain the implementation for STD and thus their results are not reported for that aggregation function. 

\begin{figure*}[t]
\vspace{-0.15cm}
    \begin{minipage}[t]{.49\textwidth}
        \centering
    	\includegraphics[width=1\textwidth]{RAQ_veraset.eps}    	    	
    	\vspace{-1.2cm}
        \caption{Time/Space/Accuracy Trade-Off on Veraset}
        \label{fig:exp:RAQ_tradeoff}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \centering
    	\includegraphics[width=1\textwidth]{res_per_epoch.eps}
    	\vspace{-1.2cm}
        \caption{Impact of training size and duration}
        \label{fig:exp:RAQ_training}
    \end{minipage}
\end{figure*}

\begin{figure}[t]
\vspace{-0.3cm}
    \centering
    \begin{minipage}{0.47\columnwidth}
    \includegraphics[width=\textwidth]{houston_pred4_visit.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\columnwidth}
    \includegraphics[width=\textwidth]{houston_pred10_visit.png}
    \end{minipage}
    %\vspace{-0.2cm}
    \caption{Learned NeuroDB with depth 5 (left) and 10 (right) for the avg. visit duration example. Color shows the visit duration in hours.}
    \label{fig:learned_query_functions}
\end{figure}

\subsubsection{Results on Veraset}\label{exp:veraset}\hfill\\
\noindent\textbf{Time/Space/Accuracy Trade-Offs}. We study different time /space/accuracy trade-offs achievable by NeuroDB and other methods, shown in Fig.~\ref{fig:exp:RAQ_tradeoff}. For NeuroDB, we vary number of layers (referred to as depth of the neural network), $d$, number of units per layer (referred to as width of the neural network), $w$, and height of the kd-tree, $h$, to see their impact on its time/space/accuracy. Fig.~\ref{fig:exp:RAQ_tradeoff} shows several possible combinations of the hyperparameters. For each line in Fig.~\ref{fig:exp:RAQ_tradeoff}, NeuroDB is run with two of those hyperparameters kept the same and another one changing. Labels of the lines can be interpreted as follows. The line labels are of the form $(height, width, depth)$, where two of \textit{height, width} or \textit{depth} have numerical values and are the constant hyperparameters for that particular line. Furthermore, the value of one of \textit{height}, \textit{width} or \textit{depth} is $\{d, w, h\}$ and is the variable hyperparameter for the plotted line. For example, line labelled (h, 120, 5) means the experiments for the corresponding line are with a NeuroDB architecture with 120 number of units per layer, 5 layers and each point plotted corresponds to a different value for the kd-tree height, and label (0, 30, d) means the experiments are run with varying depth of the neural network, with kd-tree height 0 (i.e. only one partition) and the width of the neural network is 30. The hyperparameter values are as follows. For lines (h, 120, 5) and (h, 30, 50), kd-tree height is varied from 0 to 4, for the line labelled (0, w, 5) neural network width is in the set $\{15, 30, 60, 120\}$ and for lines labelled (0, 120, d) and (0, 30, d) neural network depth is in the set $\{2, 5, 10, 20\}$. 


Finally, TREE-AGG and VerdictDB are plotted for sampling sizes of 100\%, 50\%, 20\% and 10\% of data size. For DeepDB only one result is reported since %, first, how the hyperparameters should be changed to explore the trade-offs is not discussed in \cite{hilprecht2019deepdb}, and, second, 
we observed in our experiments that changing the hyperparameters only impacts accuracy but not query time. Thus, we only report the result for the setting with the best accuracy. 


Fig.~\ref{fig:exp:RAQ_tradeoff} (a) shows the trade-off between query time and accuracy. Overall, NeuroDB performs well when fast answers are required but some accuracy can be sacrificed, while if accuracy close to an exact answer is required, TREE-AGG can perform better. Furthermore, Fig.~\ref{fig:exp:RAQ_tradeoff} (b) shows the trade-off between space consumption and accuracy. Similar to time/accuracy trade-offs, we observe that when the error requirement is not too stringent, NeuroDB can answer queries by taking a very small fraction of data size. Finally, NeuroDB outperforms DeepDB in all the metrics. Finally, comparing TREE-AGG with VerdictDB shows that, on this particular dataset, the sampling strategy of VerdictDB does not improve upon uniform sampling of TREE-AGG while the R-tree index of TREE-AGG improves the query time by orders of magnitude of VerdictDB.

Moreover, Fig~\ref{fig:exp:RAQ_tradeoff} shows the interplay between different hyperparameters of NeuroDB. We can see that increasing depth and width of the neural networks improves the accuracy, but after a certain accuracy level the improvement plateaus and accuracy even worsens if depth of the neural network is increased but the width is too small (i.e., the purple line). Nevertheless, using our kd-tree partitioning method allows for further improving the time/accuracy trade-off as it improves the accuracy at almost no cost to query time. We also observe that kd-tree improves the space/accuracy trade-off, compared with increasing the width or depth of the neural networks. This shows that our paradigm of query specialization is in fact beneficial, as learning multiple specialized models each for a different part of the query space performs better than learning a single model for the entire space.


\noindent\textbf{Median visit duration query function}. Here, we consider the query of median visit duration given a \textit{general} rectangular range. Specifically, we consider the predicate function that takes as its input coordinates of two points $p_1$ and $p_2$, that represent the location of two non-adjacent vertices of the rectangle, and an angle, $\phi$, that defines the angle the rectangle makes with the x-axis. Then, given $q=(p_1, p_2, \phi)$, the query function is to return median of visit duration of records falling in the rectangle defined by $q$. This is a common query for real-world location data, and data aggregators such as SafeGraph \cite{safegraph} publish such information.

Neither DeepDB nor DBEst can answer this query, since the predicate function is not supported by those methods, and extending those methods to support them is not trivial. On the other hand, NeuroDB can readily be used to answer this query function. Although VerdictDB can be extended to support this query function, the current implementation does not support the aggregation function, so we do not report the results on VerdictDB. Table \ref{tab:median_visit_res} shows the results for this query function. Overall, the performance of the methods is similar to other results on Veraset dataset, reported in Fig.~\ref{fig:exp:RAQ_tradeoff}.


\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c|c}
        Metric &  NeuroDB  & TREE-AGG & DeepDB & VerdictDB \\\hline
        Norm. MAE & 0.045 & 0.052 & N/A & N/A \\\hline
        Query time ($\mu s$) & 25 & 601 & N/A & N/A
    \end{tabular}
    \vspace{1pt}
    \caption{Median visit duration for general rectangles}
    \label{tab:median_visit_res}
\end{table}

\noindent\textbf{Impact of Training Size and Duration}.  Fig.~\ref{fig:exp:RAQ_training} shows the performance of NeuroDB as number of training samples and number of epochs to train changes. The results are for a NeuroDB with tree height 0 (i.e., no partitioning), neural network depth 5 and with neural network widths of 30 and 120. In Fig.~\ref{fig:exp:RAQ_training} (a), we observe that at training size of about 100,000 sampled query points, both architectures achieve close to their lowest error and further increasing number of samples only marginally improves the performance. Furthermore, when sample size is small, both architectures perform similar to each other and the neural network with larger width only starts outperforming the smaller neural network when enough samples are available. Finally, Fig.~\ref{fig:exp:RAQ_training} (b) shows that both models converge in less than one thousand epochs, for training size $5\times 10^6$ and where each epoch contains 50 batches. To reach 5000 epochs, the total training time for neural network with widths 120 and 30 was 39.7 min and 37.15 min respectively.  

\noindent\textbf{Visualizing NeuroDB}. Fig.~\ref{fig:learned_query_functions} shows the function NeuroDB has learned for our running example, for two neural networks with the same architecture, but with depths 5 and 10. Comparing Fig.~\ref{fig:learned_query_functions} with Fig.~\ref{fig:query_functions}, we observe that NeuroDB learns a function with similar patterns as the ground truth but the sharp drops in the output are smoothened out. We also observe that the learned function becomes more similar to the ground truth as we increase the number of parameters. Note that the neural networks are of size about 9\% and 3.8\% of the data size. 

%\noindent\textbf{Impact of query range on time}  Fig.~\ref{fig:exp:dist_nn_d_time} shows impact of increasing dimensionality. For larger dimensions, {ANN}'s performance deteriorates but {NeuroDB}'s performance changes by very little. Furthermore, Fig.~\ref{fig:exp:dist_nn_d_spae} shows {NeuroDB} does this by taking less space as a proportion of total data size as $d$ increases. In fact, Fig.~\ref{fig:exp:dist_nn_d_spae} shows the interesting and surprising result that neural networks with size less than actual data size are needed to calculate distance to the nearest neighbour query.  





\begin{figure*}[t]
        %\hspace{-0.5cm}
        \hspace{-0.8cm}
    \begin{minipage}[t]{.6\textwidth}
        \centering
    	\includegraphics[width=1\textwidth]{dist_nn_datasets.eps}
    	   \vspace{-0.65cm}
    	\caption{Results across datasets for NN queries}
    	\label{fig:exp:dist_nn_datasets}
    \end{minipage}
    %\hspace{-0.3cm}
    \begin{minipage}[t]{.45\textwidth}
    %\hspace*{1.8cm}
        \centering
    	\includegraphics[width=1\textwidth]{nn_dist_k.eps}
    	\vspace{-0.65cm}
    \caption{Varying $k$ for dist. NN query}
    \label{fig:exp:dist_NN}
    %\caption{Impact of $n$}
    	%\label{fig:exp:dist_nn_n_time}
    \end{minipage}
\if 0
    \begin{minipage}[t]{.24\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{exp_figs/dist_NN_error_time.eps}
    %\caption{Impact of $n$}
    	%\label{fig:exp:dist_nn_n_time}
    \end{minipage}
    \begin{minipage}[t]{.24\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{exp_figs/nn_dist_k_time.eps}
    	%\vspace{-0.7cm}
    	%\caption{Impact of $k$}
    	%\label{fig:exp:dist_nn_k_time}
    \end{minipage}
    \begin{minipage}[t]{.24\textwidth}
        \centering
    	\includegraphics[width=\textwidth]{exp_figs/nn_dist_d_time.eps}
    	%\caption{Impact of $d$}
    	%\label{fig:exp:dist_nn_d_time}
    \end{minipage}
    \fi
\end{figure*}

\subsection{Distance to $k$-th Nearest Neighbour Query}\label{sec:exp:dist_NN}
\subsubsection{Setup}
In this section, we use the NeuroDB framework with the same architecture as for RAQs to answer distance to nearest neighbour queries as defined in Sec. \ref{sec:NN}. More results on hyper-parameter tuning for distance to nearest neighbour queries and a case study on nearest neighbour queries to provide more insight into what NeuroDB learns are provided in Secs.~\ref{appx:dist_exp} and \ref{appx:NN_exp}, respectively.  % and as noted previously, it is useful for various application such as active learning \cite{settles2009active, fujii1999selective} or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour.

%\subsubsection{Setup}
\noindent\textbf{Datasets.} We use four common real datasets in our experiments whose size and dimensionality are reported in Table \ref{tab:nn_dataset_size}. For GloVe dataset, unless otherwise stated, we use the 25 dimensional version and refer by GV$<d>$ to the $d$ dimensional version of the dataset. %For each experiments, the queries are performed on the full dataset.  %the GloVe dataset \cite{pennington2014glove} that has also been used in the experiments of previous works on nearest neighbour queries \cite{zhao2020song}. The dataset contains learned word representations of about  1.2$\times 10^6$ words learned from 2$\times 10^9$ tweets. The learnt representations are available in 25, 50, 100 and 200 dimensions. 
%For each experiments, %$n$ points are sampled uniformly at random from the original dataset and are considered the database to perform the query on (the sub-sampling is done to ensure we have enough queries for training). Furthermore, 


\noindent\textbf{Query Distribution}. We assume the queries follow the data distribution, which can be true for the datasets considered. For instance, the GloVe dataset contains learned word representations. A distance to nearest neighbour query on this dataset can be interpreted as checking whether a set of words, $D$, contains a similar word to some query word $q$, or to check if a query $q$ would be an outlier in $D$ (e.g. to check whether a good representation for $q$ is learned or not). 

To generate the queries the points in the dataset are split into a training set of size $N_{train}$ and a testing set of size $N_{test}$ (points in the dataset are also training or testing queries). Unless otherwise stated, we set, $k=100$, $N_{test}=10,000$ and $N_{train}$ to the size of all the dataset except the test set. %. As discussed in \cite{glove_website}, the nearest neighbour query on word representations is semantically meaningful, as words with similar meaning are mapped close (defined by Euclidean distance or cosine similarity) to each other. A distance to nearest neighbour query on this dataset can be interpreted as checking whether a set of words, $D$, contains a similar word to some query word $q$, or to check if a query $q$ would be an outlier in $D$ (e.g. to check whether a good representation for $q$ is learned or not). 

\noindent\textbf{Measurements}. We report time taken to answer a query, space used and average \textit{relative error}. Relative error, for the $k$-th nearest neighbour query $q$, when an algorithm returns the point $p_k$ while the correct answer is $p_k^*$ is defined as $\frac{|d(p_i, q)-d(p_i*, q)|}{d(p_i*, q)}$, where $d(x, y)$ is the Euclidean distance between $x$ and $y$. Furthermore, since the KDD dataset contained near duplicate records, the distance to the nearest neighbour could be very close to zero and relative error could be very large for small absolute error values. Thus, only for this dataset, we present the results for normalized mean absolute error (as defined in Sec.~\ref{sec:exp:rang_agg}) instead of relative error. 
%(we assume no point is the nearest neighbour of itself to avoid $d(p_i*, q)=0$). 
%We set our error requirement to $0.05$ and for all the methods, present the lowest query time such that their relative error is at most $0.05$. We also study the trade-off between accuracy and query time, the results of which are reported in our technical report \cite{techreport}.

\noindent\textbf{Baseline Algorithms}. We compare our algorithm with {NSG} \cite{fu2017fast} and {ANN} \cite{arya1998optimal}. {NSG} is a state-of-the-art graph-based algorithm, shown in \cite{fu2017fast} to outperform various existing methods. We use their publicly available implementation \cite{nsg_imp}. We also use {ANN} which is a wort-case optimal algorithm %(in the algebraic decision tree model of computation as it requires $O(n)$ space and $O(\log n)$ query time for fixed, $d$, $\epsilon$ and $k$ \cite{arya1998optimal}), 
as implemented in ANN library \cite{ann_lib}. The algorithm, given a worst-case relative error parameter, $\epsilon$, returns $k$ nearest neighbours of $q$ such that the relative error for the $k$-th nearest neighbour in $D$ is at most $\epsilon$. For both methods to select algorithm parameters, we perform a grid search to find the parameters such that the query time is minimum while relative error is around 0.05.  

%We use the grid search method discussed in \cite{fu2017fast} to select the parameters algorithm parameters. For each dataset, we perform a grid search on the hyper-parameters to find the parameters such that the query time is minimum while relative error is around 0.05.   . In our experiments, we report the query time of {ANN} where average relative error is at most some threshold, e.g. 0.05. Since {ANN} takes \textit{worst-case} relative error as an input (and not \textit{average} relative error), we need to find a value for the worst-case relative error such that average relative error is below 0.05. To do this, we perform a binary search on values for worst-case relative error until we find a value such that the average relative error is below 0.05.



%\vspace{-0.4cm}
\subsubsection{Comparison Across Datasets}\label{sec:exp:dist_NN_res}
%\noindent\textbf{Results on different datasets}. 
Fig.~\ref{fig:exp:dist_nn_datasets} shows the results on different datasets for both distance to $k$-NN and $k$-NN queries. Note that for the baseline algorithms, the error and query time for answering both $k$-NN and distance to $k$-NN is the same, since the algorithms, in both cases, return $k$ nearest neighbours as their output. In the figure, NeuroDB (dist) is NeuroDB trained to answer distance to $k$-NN queries and NeuroDB (NN) is trained to answer $k$-NN queries. Furthermore, we implemented NeuroDB (NN)+NSG, which is an algorithm that takes the output of NeuroDB (NN), and finds its first nearest neighbour in the database using NSG.  

\noindent\textbf{Distance to $k$-NN}. First, observe that NeuroDB is able to answer distance to $k$-NN queries orders of magnitude faster than the state-of-the-art while achieving similar accuracy. Furthermore, its query time is only marginally affected by data dimensionality (e.g., see GV25 to GV200 results) and changes very little for datasets with different sizes. We emphasize that these results are obtained without any parameter tuning for NeuroDB, and NeuroDB's architecture is exactly the same as when performing RAQs. This shows that NeuroDB can be applied to two different query types with minimal effort, and thus, can save time when designing a system.   % $n$ increases while there are significant changes in the other algorithms. We note that theory suggest that {ANN} has logarithmic query time in $n$ given a fixed \textit{worst-case} error \cite{arya1998optimal}. However, in practice, we observe that we need to change maximum error depending on data size to keep average error constant. 

\noindent\textbf{$k$-NN}. Fig.~\ref{fig:exp:dist_nn_datasets} also shows the results for $k$-NN queries. Note that the output of NeuroDB (NN) is a $d$-dimensional point, but the point is not necessarily in the dataset. Thus, even though Fig.~\ref{fig:exp:dist_nn_datasets} shows that NeuroDB (NN) can answer $k$-NN queries with accuracy similar to NSG but much faster for high dimensional datasets, such an answer may not be useful for real-world applications. Thus, we investigated using NSG together with NeuroDB (NN). Such an algorithm first runs NeuroDB (NN), and then runs NSG to find the nearest neighbour of the output of NeuroDB (NN). Intuitively, this can improve query time because NeuroDB (NN) is very fast, and NSG only needs to find the first nearest neighbour instead of $k$-th nearest neighbour. We observe that, for high dimensional datasets, such an algorithm can improve the query time over standalone NSG while obtaining similar accuracy. Thus, such a hybrid approach can be useful, where NeuroDB is used as a heuristic to search the space, but we leave a full investigation of such hybrid approaches to the future work.

\subsubsection{Impact of $k$ on GloVe dataset}\label{sec:exp:dist_NN_glove}
%\noindent\textbf{Impact of $n$ and $d$}.  Fig.~\ref{fig:exp:dist_NN} (a) and (b) shows impact of increasing data size and dimensionality. For larger size and dimensions, NSG and {ANN}'s performance deteriorates but {NeuroDB}'s performance changes very little and NeuroDB outperforms them by more than an order of magnitude when $d=200$ or when $n=160,000$. Furthermore, for the sake of space, in our techincal report \cite{techreport}, we present the results on space used by NeuroDB, which shows NeuroDB achieves this by taking size less than 50\% of the actual data size.  %\noindent\textbf{Impact of $k$ on query time}. 
Fig.~\ref{fig:exp:dist_NN} shows how changing $k$ impacts the performance. Overall $k$ has no impact on query time of {NeuroDB}, because for any value of $k$ the cost of using {NeuroDB} is just a forward pass of the neural network. However, {NSG} and {ANN} need to find all the $k$ nearest neighbours, and thus their performance deteriorates with $k$. Better support for larger values of $k$ is one of our motivations for using {NeuroDB}, as it can find the distance to $k$-th nearest neighbour without unnecessarily finding all $k$ nearest neighbours, which other methods do.




\if 0
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
        Algorithm & count & mean & std  \\\hline
        {NeuroDB} & 27.26 & 27.26 & 27.26\\\hline
        {ON-AGG} & 1,644 & 1,055  & 1,017
    \end{tabular}
    \caption{Query time ($\mu s$) for $n=100,000$ and $d=2$}
    \label{tab:comparison}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
        Algorithm & count & mean & std  \\\hline
        {NeuroDB} & 27.26 & 27.26 & 27.26\\\hline
        {DBEst} & 27.26 & 27.26 & 4,629\\\hline
        {ON-AGG} & 1,644 & 1,055  & 1,017
    \end{tabular}
    \caption{Query time ($\mu s$) for $n=100,000$ and $d=2$}
    \label{tab:comparison}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
        Algorithm & count & mean & std  \\\hline
        {NeuroDB} & 0.015 & 0.017 & 0.015\\\hline
        {ON-AGG} & 1,644 & 1,055  & 1,017
    \end{tabular}
    \caption{Normalized MSE for $n=100,000$ and $d=2$}
    \label{tab:comparison}
\end{table}
\fi






==> NeuroDB-ICDE (tech)/Introduction.tex <==
\vspace{-0.1cm}
\section{Introduction}
\vspace{-0.1cm}
Range aggregate queries (RAQs) are an integral part of many real world applications. Calculating the total profit over a period from sales records or the average pollution level for different regions for city planing \cite{ma2019dbest} are examples of their use cases. Often, due to large volume of data, an exact answer takes too long to compute and a fast approximate answer is preferred. In such scenarios, there exists a time/space/accuracy trade-off, where algorithms can sacrifice accuracy for time or space. For example, consider a geospatial database containing latitude and longitude of location signals of individuals and, for each location signal, the duration the individual stayed in that location. A potential RAQ on this database is to calculate the average time spent by users in an area, which can be useful for analyzing different Points of Interest (POIs). Approximate answers within a few minutes of the exact answer can be acceptable in such applications. We use such a scenario as our running example, with the database shown in Fig. \ref{fig:visit_query_function} (left).

Research on RAQs has focused on improving the time/space/accuracy trade-offs.
%Answering RAQs has been studied for decades , with the goal of improving the time/space/accuracy trade-offs. 
Existing methods can be divided into sampling-based \cite{hellerstein1997online, agarwal2013blinkdb, chaudhuri2007optimized, park2018verdictdb} 
and model-based methods \cite{graham2012synopses, schmidt2002propolyne, ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. Sampling-based methods sample a subset of the database %according to a sampling strategy,  (e.g., uniform sampling, \cite{hellerstein1997online}, stratified sampling \cite{chaudhuri2007optimized, park2018verdictdb})
and answer the queries based on the samples. Model-based methods develop a model of the data to answer the queries. Models can be of the form of histograms, wavelets and data sketches (see \cite{graham2012synopses} for a survey). More recently, learning-based regression and density data models \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb} were proposed which have shown improvements over existing techniques. %Generally, the model-based approached follow two steps. First, a model of the data is created. Then, a method is proposed to use these data models to answer the queries..

A major drawback of the recent learning-based approaches is that they learn a model from the data that is oblivious to the queries being asked. Learning from the data misses the opportunity to learn information about the queries that can help answer them faster. This information can be of two forms. (1) It can be about the query workload. In real-world databases, certain queries are far more common than others. In fact, OLAP systems (e.g., \cite{oracle, tableau}) divide attributes into \textit{measure} and \textit{dimension} categories where common RAQs have an aggregation function on a \textit{measure} attribute and range predicates on \textit{dimension} attributes. In our running example, visit duration can be defined as a measure attribute and lat. and lon. as dimension  attributes. Other queries, such as the query of average latitude given a visit duration range may not make any semantic sense. Even given the measure and dimension attributes, some ranges are queried more often than others. In our running example, more RAQs may be asked in downtown vs. a residential area. Diverting model capacity to learn about the queries that will actually be asked can improve the performance of a system. (2) The information can also be about the patterns in the answer to the query. The average visit duration for different places in the downtown of a city may be similar, while the answer will be different for suburban areas. A model can find such patterns, so that a compact representation of the data \textit{relevant to the queries} is learned.


%This negative influences learning of this approach on learning can be seen from two angles. First, the query learning process is oblivious to the query workload. That is, a  

\begin{figure}
    \centering
    \begin{minipage}{0.47\columnwidth}
    \includegraphics[width=\textwidth]{db_houston.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\columnwidth}
    \includegraphics[width=\textwidth]{houston_true_visit.png}
    \end{minipage}
    \caption{Running example: (left) Database of location signals, and (right) the query function of average visit duration. Color shows visit duration in hours.}
    \label{fig:visit_query_function}
\end{figure}
\vspace{-0.1cm}
\subsection{NeuroDB for Range Aggregate Queries}\label{sec:intro:neurodb_RAQ}
\vspace{-0.1cm}
We propose a fundamentally different approach towards answering RAQs. First, we introduce the notion of a \textit{query function}. Intuitively, a range aggregate \textit{query function} takes as an input a range predicate and outputs a real number, which is an aggregation of a measure attribute. In our running example, consider the query of average visit duration for a 50m$\times$50m rectangle with bottom left corner at the geo-coordinate $(x, y)$. For such an RAQ, a query function, $f_D(x, y)$, can be defined that takes as input the geo-coordinate of the rectangle and outputs the average visit duration of data points in the rectangle. This query function is plotted in Fig.~\ref{fig:visit_query_function} (right). We call a particular input to the query function a \textit{query instance}. For example, Fig.~\ref{fig:visit_query_function} (right) shows that for query instance (-95.3615, 29.758) the answer is 9, i.e., $f_D(-95.3615, 29.758)=9$. %\footnote{We use \textit{query instance} and \textit{query function} terminologies to distinguish between a particular query input (instance) and the general relationship between query inputs and their corresponding outputs (function).} and can be seen as a function mapping the \textit{query space} to some \textit{output space}. 

The observation that RAQs can be represented as query functions allows us to learn models to answer them efficiently. To that end, we propose a novel framework, called \textit{Neural Databases} (NeuroDB), to efficiently answer RAQs. Specifically, let $q$ be a query instance issued by a user, and let $f_D(x)$ be the range aggregate query function, defining what the answer is for any query instance $x$ (and thus the ground truth answer for $q$ is $f_D(q)$). During a pre-processing step, NeuroDB uses solved query instances from a known algorithm to learn a model that approximates the query function well. %In this step, NeuroDB uses solved query instances from a known algorithm to train a model, $\hat{f}_D(x;\theta)$, that approximates the query function well. 
The model takes a query instance as an input and outputs an answer, and the training objective is to optimize the model so that its answer is as close to ground truth as possible. At test time, NeuroDB outputs $\hat{f}_D(q;\theta)$ as its answer for query $q$, \textbf{eliminating both the database and the algorithm it learned from}. In our running example, NeuroDB learns a model that looks similar to Fig.~\ref{fig:visit_query_function} (right), but can be evaluated fast and without accessing the database at all. We use neural networks as our model and propose a neural network architecture that can be easily trained, answer the queries fast and accurately, and scale with dimensionality and data size.


%To answer this query type, we can learn a model (or function approximator) that approximates the specific query function, where the model takes as input a range predicate and outputs a real number. Different models can be trained for different query functions, each optimized for the specific query. %An approximation algorithms can be seen as functions approximating the query function, or, in other words, as \textit{function approximators}.   


%We propose a novel framework, called \textit{Neural Databases} (NeuroDB), to efficiently answer range aggregate queries. By viewing database queries as functions, we propose a neural network framework that can approximate the query function well. Specifically, for a database, we consider range aggregate query functions of interest for which efficient answers are desired, e.g., the query of average visit duration for a particular location. Then, for each such query function, 

%We use neural networks as our function approximator. Neural networks can learn patterns in the real-world data and the relationship between query input and output, which means small models can answer queries well. They can be trained for specific query distributions, which allows more accurate modeling for the distribution and avoiding redundancies. In fact, NeuroDB can be seen as an approximate result materialization technique, where regions with higher probability in the query space are materialized more accurately. Furthermore, neural networks' architecture can be adjusted to learn complex queries and thus they can be applied to different domains with varying difficulty. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction. %Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section
%The neural network then can be used to replace the database for answering the queries. Our framework is simple and query-type agnostic, that is, it makes no assumption about the query type learned, and yet can provide orders of magnitude performance gains for the specific queries. We use neural networks to be able to capture the complex relationships that can exist between query inputs and outputs. 
%However, designing a neural network architecture that can be easily trained, can answer the queries fast and accurately, and can scale with dimensionality and data size is not straightforward. We propose a novel architecture that achieves all of these objectives. 

NeuroDB improves the state-of-the-art in two ways. First, we experimentally observed that NeuroDB answers RAQs multiple orders of magnitude faster than state-of-the-art and with better accuracy. Thus, in traditional data management systems, NeuroDB can be an addition to the query processing engine and can considerably improve the performance of RAQs, while a default query processing engine can answer queries for which NeuroDB is not trained. In this regard, NeuroDB can be used similar to how indexes are used in database systems. Second, NeuroDB trained for a query function is typically much smaller than data size, while the model learned can be used to answer the queries without accessing the data. This is beneficial for applications requiring efficient release and storage of data. For instance, location data aggregators (e.g., SafeGraph \cite{safegraph}) can train NeuroDB to answer the average visit duration query, and release it to interested parties instead of the dataset. This can improve the storage, transmission and query processing costs for all parties. % involved. 

%From another perspective, NeuroDB can be seen as an approximate result materialization technique that takes advantage of query and data distribution to minimize the approximation error. Roughly speaking, regions with higher probability in the query space are materialized more accurately, allowing the framework to perform well for high-dimensional data such as images where queries can be seen as belonging to low dimensional manifolds \cite{roweis2000nonlinear, chen2018sparse}. Intuitively, NeuroDB can be thought of as \textit{memorizing the data points} in the model weights. Although no general guarantee exists that this memorization should take less space than the actual data, in practice, we observe that due to the existence of patterns in the data and the relationship between query input and output, NeuroDB can answer queries by only taking up a fraction of the data size (and without the need to access the database). We note that this is different from merely \textit{memorizing or caching the answers to query points} in the training set, as we experimentally show that NeuroDB learns generalizable patterns between query input and output.

%Overall, in a database system, the choice of what range aggregate queries NeuroDB should be trained to answer is akin to the question of which attributes should be indexed.   


\subsection{Beyond Range Aggregate Queries}\label{sec:intro_NN}
Our observation that queries can be represented by query functions is not specific to RAQs, and is true for any query type. Considering such representation opens the path for using learned models to answer different database query types. Hence, an important question is to understand the utility of learned models for different query types. We take the first step in this direction by applying NeuroDB to another query type. Specifically, we consider two variants of $k$-th nearest neighbour queries. This is possible because the training of NeuroDB is query type agnostic, that is, it does not make assumptions about the query type during training. 

First, we consider $k$-th nearest neighbour queries ($k$-NN), which, for a $d$-dimensional database $D$, can be represented by a function, $f_D^{NN}(.)$ that takes a $d$-dimensional point as an input, and outputs another $d$-dimensional point. NeuroDB can be used to train a model, $\hat{f}_D^{NN}(.;\theta)$ that mimics the function $f_D^{NN}(.)$. We observed that NeuroDB can provide an answer for the $k$-NN query that is spatially close to the true answer. However, for a query $q$, the output of $\hat{f}_D^{NN}(q;\theta)$ is not necessarily in the database (but rather some point in $\mathcal{R}^d$ whose distance to $f_D^{NN}(q)$ is small), while the answer to nearest neighbour query needs to be a point in the database. %That is, NeuroDB is able to provide an answer that is similar to the $k$-th nearest neighbour of a query point, but not an answer that is in the database $D$. 
Such an answer may not have much utility in real-world applications. %Nonetheless, the fact that NeuroDB is able to answer approximately where the $k$-th nearest neighbour can be useful as a heuristic for searching the space. Our experiments show that using NeuroDB together with a state-of-the-art algorithm for nearest neighbour queries can provide performance gains in high-dimensional datasets.}

%Applying NeuroDB to this query type, we experimentally observed that answering such a query requires very large neural networks, which does not provide any benefit in terms of query or storage cost compared with existing methods. 

Next, we consider the \textit{distance to} $k$-th nearest neighbour query, where the query answer is the distance to and not the actual point in the database. This query can be represented by a function that takes a $d$-dimensional query point as an input and outputs a real number. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (e.g., as a diversity score for selecting samples for training a model), outlier detection \cite{chandola2009anomaly} and assessing probability of getting infected from a disease (e.g., COVID-19) calculated based on proximity to the nearest infected person. We observed that NeuroDB is able to answer distance to $k$-NN queries orders of magnitude faster than state-of-the-art, while only taking space that is a small fraction of data size. NeuroDB achieves this because %, in contrast to existing methods, 
it answers distance to $k$-NN queries without calculating any distances or finding any of the neighbours at query time. %Contrasting this with existing methods that need to find the $k$-th nearest neighbour to calculate distance to $k$-th nearest neighbour shows the advantage of NeuroDB that it can provide answers for specific queries without unnecessary precomputations. 
%
Instead, NeuroDB approximately materializes the query results, with higher probability regions (according to query distribution) being materialized more accurately. This allows the framework to perform especially well for high-dimensional data where queries are from a small portion of the total high dimensional space (e.g. images\cite{roweis2000nonlinear}).
%such as images where queries can be seen as belonging to low dimensional manifolds \cite{roweis2000nonlinear, chen2018sparse}.
%
%Furthermore, NeuroDB avoids curse of dimensionality by learning from the query distribution. An exact materialization of 
%
%4For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because potential queries can be a small proportion of the total high dimensional space (e.g. for images). %This is in contrast to .  (e.g., finding the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. %without Although distance to $k$-NN queries is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

The results in this paper suggest dividing database queries into \textit{item queries} and \textit{statistic queries} categories. Item queries are queries where the answer is an actual database item, while statistic queries are queries where the answer is a numerical statistic calculated based on the database. We conjecture that NeuroDB, on its own, is useful for statistic queries. Studying this conjecture for different statistic queries is an interesting future research direction, where a generic framework can be used to answer multiple different query types in this category. This paper is a first step in that direction, where a framework designed for range aggregate queries is shown to also efficiently answer distance to the $k$-th nearest neighbour queries and outperform the state-of-the-art for both of them. Although NeuroDB outperforming the state-of the-art in either of the two query types is significant on its own, this paper also sheds light on the possibility that a learned framework can be generalizable to multiple query types. As such, it can improve the performance of a system while also saving time when designing it. For item queries, NeuroDB may be useful as part of other algorithms designed for such queries, the study of which we leave for future work.


%The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%Searching the algorithm space translates into searching for good parameters of (or, in other words, learning) a function approximator. In this paper, as an initial attempt, we restrict the algorithm space to the set of parameters of a neural network because it can be searched efficiently. Therefore, we formalize the problem of using learned function approximators to answer database queries and show that, for the specific query types of distance to nearest neighbour query and range aggregate query, a learned neural network can provide better time/space/accuracy trade-offs than existing methods in practice. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction.%Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section


%Although the NeuroDB framework is query-type agnostic, and as such, can be applied to any query type, in this paper, we only show that it specifically provides orders of magnitude improvement for range aggregate queries and distance to nearest neighbour query. We do not make any claim about its efficiency for other query type. However, due to its good performance for the considered query types, we conjecture that NeuroDB can also be applied to other query types efficiently, but we leave studying this claim for the future work. Nevertheless, both queries considered in this paper are important building blocks of many real-world systems. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (for instance, it can be used as a diversity score for selecting samples for training a model) or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. Although it is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

%\noindent\textbf{NeuroDB vs. Combinatorial Methods}. To contrast NeuroDB with existing combinatorial methods, we note that (1) NeuroDB avoids curse of dimensionaity by utilizing the query distribution. For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all potential queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because the space of potential queries can be a small proportion of the total high dimensional space (e.g. for images). (2) NeuroDB can provide answers for specific queries without unnecessary precomputations. For instance, a model can be trained to find the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. 
%(3) Parallelization of NeuroDB is the problem of performing a forward pass of a neural network in parallel, is a well-studied problem [XX] and does not depend on the query type. 
%(3) NeuroDB uses query and data distribution to learn patterns that allow for answering queries faster. (4) The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%\noindent\textbf{NeuroDB vs. Machine Learning Methods}. Machine learning methods have been used to solve various combinatorial problems such as TSP, Max cut, etc \cite{li2018combinatorial, khalil2017learning, nazari2018reinforcement}. This paper extends those works to answering generic database queries using neural networks. Answering specific database queries using machine learning has been studied in the literature, such as for indexing \cite{kraska2018case, galakatos2018tree, ding2019alex} and specific aggregate queries \cite{hilprecht2019deepdb, ma2019dbest}. These methods have shown promise in the area they have been applied to, with their success being attributed to the ability of the models to learn and utilize the data and/or query distributions. The main observation in these bodies of work is that a certain database operation (e.g. getting the location a record is stored  for the case of indexing in \cite{kraska2018case}) can be replaced by a learned model. In this paper, we observe the overarching idea that, in fact, answering \textit{any} query can be done by a model, since any query is a function that can be approximated. Using this observation, we show that small, multi-layer neural networks can efficiently and accurately answer range aggregate queries and distance to nearest neighbour queries, improving on the modeling choices of the previous work and the state-of-the-art in the studied query types. %In this respect, our work can be seen as a generalization of the recent work in this area. The advantage in our framework is that it can be applied to different query types. %. However, no framework has been proposed that is able to answer different query types, i.e., both nearest neighbour and range aggregate queries efficiently. Furthermore the proposed techniques use basic regression models [X], while we show how the expressive power of multi-layer neural networks can be utilized.


\subsection{Contributions and Roadmap}
%\noindent In this paper, we 
\begin{itemize}[leftmargin=10pt]
        \item We formulate the problem of learning RAQs with function approximators (Sec. \ref{sec:def}); 
        \item Propose NeuroDB, the first neural network framework to answer RAQs efficiently  (Secs. \ref{sec:NeuroDB}, \ref{sec:raq_extension}); and
        \item Show how NeuroDB can also answer distance to nearest neighbour queries (Sec. \ref{sec:NN}).
        \item Our experiments show that
        \begin{enumerate}[leftmargin=4pt]
            \item {NeuroDB} enjoys orders of magnitude gain in query time and provide better accuracy over state-of-the-art for answering RAQs using real-world, TPC-benchmark and synthetic datasets (Sec.~\ref{sec:exp:rang_agg}); and
            \item The same architecture is used to answer distance to nearest neighbour query with orders of magnitude gain in query time over state-of-the-art on real datasets. NeuroDB's query time is not affected by $k$ and only marginally impacted by data dimensionality (Sec. \ref{sec:exp:dist_NN}).
            %\item As a byproduct, we show that {NeuroDB} can learn patterns in the data, and thus is useful for feature learning or when there is missing data (Sec. \ref{sec:exp:NN}).  
        \end{enumerate}
        \end{itemize}
\noindent Sec.~\ref{sec:related_work} presents related work and we conclude in Sec.~\ref{sec:conclusion}.

%Thus, our method is not applicable for NP-hard queries where collecting samples is difficult. 

%State the problem we're trying to solve: fast solution/not a lot of updates/low dimensional answer. Other examples of low dimensional query

\if 0

\begin{itemize}
    \item \textbf{Motivation}
    \begin{enumerate}
        \item Need for fast query processing, can sacrifice accuracy
        \begin{itemize}
        \item Running Examples: 
        \item (Distance to nearest neighbour query): distance-based outlier detection in video streams, or selecting video frames that are different enough from current samples for training. Want to analyze fast enough to process the stream on the fly
        \item (Range aggregate queries): Calculating avg. pollution level over time and regions for city planing \cite{ma2019dbest}. Large dataset, so exact solution takes too long, but error is acceptable
        \end{itemize}
        \item A lot of Human time is spent on designing efficient algorithms to answer queries
        \begin{itemize}
            \item Example: Different algorithms are designed for answering nearest neighbour queries, range aggregate queries, skyline queries, etc. 
            \item The algorithms are specific to queries
            \item So need to spend a lot of time designing new algorithms for new queries 
        \end{itemize}
    \end{enumerate}
        \item \textbf{Existing Solutions}
        \begin{itemize}
            \item Combinatorial Methods: Calculate answers by an algorithm that accesses the data
            \begin{itemize}
                \item Curse of dimensionality
                \begin{itemize}
                    \item Performance degrades with dimensionality
                    \item Neural network based dimensionality reduction methods are often used
                \end{itemize}
                \item Unnecessary calculations
                \begin{itemize}
                    \item We might only need distance to 100-th nearest neighbour (e.g. for distance based outlier detection), but need to find all the 100 nearest neighbours
                \end{itemize}
                \item Hard to parallelalize
                \item Combinatorial solutions aren't general
                \begin{itemize}
                    \item Hard/time-consuming to design new fast combinatorial method for new queries, or automate the process of designing algorithms
                    \item No combinatorial method can handle \textit{all} queries fast
                \end{itemize}
            \end{itemize}
            \item Learning-based methods
            \begin{itemize}
                \item Have been successfully applied to some database/combinatorial problems
                \item But no general neural network-based framework for learning
            \end{itemize}
        \end{itemize}


    \item \textbf{Neural Databases}
    \begin{itemize}
        \item Overview
        \begin{itemize}
            \item Database queries are functions
            \item Learn from sample queries and their answer
            \item Answer queries without data access
        \end{itemize}
        \item General method for answering any query approximately
        \item Takes advantage of data/query distribution
        \item Can be applied to any query
        \begin{itemize}
            \item The framework is general, but we show that it can be applied to queries with low-dimensional outputs
            \item higher-dimensional output needs more training samples to avoid over-fitting so are harder to learn
        \end{itemize}
        \item Scales easily with more computational power
        \item Differentiable database operations (possible applications in ML)
    \end{itemize}
    \item Neural Database vs. ML for combinatorial optimization
    \begin{itemize}
        \item Answers different queries on a particular database, compared with answering different instances of a problem type
    \end{itemize}
    \item Neural Database vs. existing ML use-cases for DB problems
    \begin{itemize}
        \item Ad-hoc ML use-cases, no general framework applicable to all problems
        \item Indexing \cite{kraska2018case} and aggregate queries \cite{ma2019dbest} are special cases
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item View of database queries as functions that can be learned
        \item Propose first general framework to answer queries efficiently using neural networks
        \item Design a model based on the framework
        \item Show how it can be applied to nearest neighbour/distance to nearest neighbour/range aggregate queries
        \item Experimentally show it does better than existing methods
    \end{itemize}
\end{itemize}

\fi

==> NeuroDB-ICDE (tech)/Introduction_old.tex <==
\section{Introduction}
Range aggregate queries are a building block of various real world applications, from calculating total profit over a period from sales records to calculating average time spent by users in an area in a geo-spatial database. Often, exact answers are not required and an approximate but fast answer is preferred. For instance, an exact answer to the range aggregate query of calculating average pollution level for different time periods and regions for city planing \cite{ma2019dbest} may take too long due to large volume of data, but an approximate answer may be as valuable. In such scenarios, there exists a time/space/accuracy trade-off, where algorithms can sacrifice accuracy for time or space. 

Answering range aggregate queries has been studied for decades in the area of approximate query processing \cite{chaudhuri2017approximate}, where the goal is to improve upon the time/space/accuracy trade-off. Broadly speaking, the methods can be divided into sampling-based methods \cite{hellerstein1997online, agarwal2013blinkdb, chaudhuri2007optimized, park2018verdictdb} 
and model-based methods \cite{graham2012synopses, schmidt2002propolyne, ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. Sampling-based methods randomly sample a set of points from the database according to a sampling strategy, % (e.g., uniform sampling, \cite{hellerstein1997online}, stratified sampling \cite{chaudhuri2007optimized, park2018verdictdb})
and answer the queries based on the samples.  Model-based methods develop a model of the data that is used to answer queries. The models can be of the form of histograms, wavelets, data sketches (see \cite{graham2012synopses} for a survey) or, more recently, regression and density based models \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. %Generally, the model-based approached follow two steps. First, a model of the data is created. Then, a method is proposed to use these data models to answer the queries. 
Recent work \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}  has used machine learning and different modeling choices have been proposed to learn the data distribution. These studies show that modelling the data using machine learning techniques improves the accuracy over existing sampling-based techniques.

While the machine learning models have been successful, the modelling choices can be improved substantially. We first discuss three design principles that we utilize to improve upon the state-of-the-art in this paper. 

\noindent\textbf{Not All Queries Are Equal}. In real-world databases, certain queries are far more common than others. For instance, in a geo-spatial dataset containing latitude and longitude of visits of individuals to a location, together with the visit duration, a common range aggregate query consists of a range predicate on the location with the average aggregation function on the visit duration (while, e.g., the query of average latitude given a visit duration predicate may not make any semantic sense). For such frequent queries, speeding up the computation can improve the performance of the system.  However, the query distribution is ignored in recent machine learning methods \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb} for answering range aggregate queries. %Existing work misses the opportunity to learn information about the common queries that can help answering them faster.

\noindent\textbf{Query Specialization}. Modelling the data, as done in \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}, does not use any query specific information in learning. The model learnt is oblivious to the queries being asked. An alternative to modelling the data and using that model to answer all different queries is to learn specialized models for specific queries. Using query specialized models, different models are learned to answer different queries. For instance, in the geo-spatial dataset example, a model can be learned that is trained to answer queries with a range predicate on location and average aggregation function on visit duration.  Intuitively, a model specialized for a specific query (e.g., for specific range predicates and aggregation function and attribute) can answer the query more accurately and faster than a single model of the entire data, because the model only needs to learn the relevant information from the data to that particular query. Furthermore, given that in real-world datasets, not all possible queries are typically asked (or are meaningful, as mentioned in the paragraph above) the learned model can include less redundant information compared with the data. Nevertheless, multiple query-specialized models may consume more space than a single data model, but, even in that case, the space consumption is traded for better query time and accuracy, extending the set of achievable time/space/accuracy trade-offs. 

\noindent\textbf{Queries Are Functions}. Finally, we observe that range aggregate queries can be thought of as functions that can be approximated. This observation allows us to learn a specialized model, trained to answer a specific range aggregate query. Particularly, a \textit{query type} (or a \textit{query function}) on a database defines what the output should be for a \textit{query instance}\footnote{We use \textit{query instance} and \textit{query function} terminologies to distinguish between a particular query input (instance) and the general relationship between query inputs and their corresponding outputs (function).} on the database and can be seen as a function mapping the \textit{query space} to some \textit{output space}. For instance, in the geo-spatial database example, the input to the function is a range predicate and the output is a value in $R$. To answer this query type, we can learn a model (or function approximator) that approximates the specific query function, where the model takes as input a range predicate and outputs a real number. Different models can be trained for different query functions, each optimized for the specific query. %An approximation algorithms can be seen as functions approximating the query function, or, in other words, as \textit{function approximators}. 



%Answering database queries fast, with low storage cost and high accuracy are important performance goals in a database system. A general trade-off exists between these metrics, e.g., query time can be improved by increasing space consumption or sacrificing accuracy. In some applications, exact answers are not required and an approximate but fast answer is preferred. For instance an exact answer to the \textit{range aggregate query} of calculating average pollution level for different time periods and regions for city planing \cite{ma2019dbest} may take too long due to large volume of data, but an approximate answer may be as valuable. Many other scenarios where approximate answers to queries are acceptable are considered in the literature \cite{chaudhuri2017approximate}. Another example is distance-based outlier detection \cite{chandola2009anomaly} on a video stream, or selecting video frames for training a vision model \cite{settles2009active, fujii1999selective} from a video stream that requires algorithms that compute  \textit{distance to the $k$-th nearest neighbour} of the frames of a video stream over an existing database of images on the fly. The need for fast answers is often aggravated by the limitations of the device performing the computation. IoT and edge devices with limited processing/storage capacity are being utilized more often to capture videos and perform these operations \cite{qian2019active, Yang2018active}. Accuracy can be sacrificed for faster query response time to allow for processing of more video frames.  We primarily focus on range aggregate queries and distance to nearest neighbour queries which are two important underlying query types for which approximate answers are acceptable.

%\noindent\textbf{Grand Vision}. Another less-studied aspect of designing algorithms for different queries is the limitations and downsides of manually designed algorithms. In addition to the human time spent on designing efficient algorithms which could be saved, distribution of the data points and the query points are not fully exploited and the set of potential solutions is limited to human imagination and throughput. An automated framework that can efficiently answer range aggregate queries and distance to nearest neighbour queries,  and other, potentially new or application specific, types of queries is ideal. \textit{This paper is our first step towards the ultimate goal of devising a system that can automatically search an algorithm space to find algorithms with better time/space/accuracy trade-offs for different query types}, where an algorithm space is a set of potential algorithms that answer a query. 


%the human time spent on designing efficient algorithms, and the limitations of manually designed algorithms. Nearest neighbour queries are studied separately \cite{friedman1975algorithm, guan1992equal, bei1985improvement} from range aggregate queries \cite{graham2012synopses, hellerstein1997online, park2018verdictdb, ma2019dbest}, and several customized \textit{query-specific} algorithms have been developed to answer them efficiently. The large space of potential algorithms is manually explored by human experts to improve upon time/space/accuracy of the algorithms for different query types. However, no automated solution has been studied that can be applied to different query types. 

%\noindent\textbf{First Step}. Our first step towards that goal, presented in this paper, consists of

%We approach the problem by designing a framework that can learn an algorithm for one query type, namely, range aggregate queries, and showing that the same framework can be used to learn an algorithm for another query type, namely distance to the $k$-th nearest neighbour query, while outperforming the stat-of-the-art for both of them. Although an algorithm outperforming the state-of the-art in either of the two query types is significant on its own, our goal in this paper is to show that a learned framework can not only be useful for a specific query type, but can be generalizable to multiple query types (specifically query types that are traditionally studied separately, e.g., nearest neighbour queries and range aggregate queries). As such, it can improve the performance of a system while also saving time when designing it.

%To that end, in this paper, we make the observation that queries can be thought of as functions that can be approximated. This allows us to formulate a learning task, i.e., to learn a model, to answer a query. To be specific, a  \textit{query type} (or a \textit{query function}) on a database defines what the output should be for a \textit{query instance}\footnote{We use \textit{query instance} and \textit{query function} terminologies to distinguish between a particular query input (instance) and the general relationship between query inputs and their corresponding outputs (function).} on the database and can be seen as a function mapping the \textit{query space} to some \textit{output space} (e.g., for the nearest neighbour query on a $d$-dimensional database, query space is all the points in $R^d$ and output space is all the points in the database). Algorithms can be seen as functions approximating the query function, or, in other words, as \textit{function approximators}. This observation, generalizes ``Indexes are models'' of \cite{kraska2018case} to \textit{queries are functions that can be approximated}. %In \cite{kraska2018case}, traditional B-tree \cite{bayer2002organization} is replaced by a learned index. Our work can be seen as a generalization of their idea, where any query function can be replaced by a learned function approximated. 
%Using this terminology, where any algorithm is seen as a function approximating a query function\footnote{the approximation error is zero in many cases, e.g. for B-trees.}, we can say that a traditional B-tree \cite{bayer2002organization} as well as RMI \cite{kraska2018case} approximate an index query function, nearest neighbour query function can be approximated by combinatorial methods such as \cite{friedman1975algorithm, guan1992equal, bei1985improvement} and range aggregate query function by \cite{graham2012synopses, hellerstein1997online, park2018verdictdb}. 

\subsection{NeuroDB for Range Aggregate Queries}
We propose a novel framework, called \textit{Neural Databases} (NeuroDB), to efficiently answer range aggregate queries. By viewing database queries as functions, we propose a neural network framework that can approximate the query function well. Specifically, for a database, we consider range aggregate query functions of interest for which efficient answers are desired, e.g., the query of average visit duration for a particular location. Then, for each such query function, during a pre-processing step, NeuroDB learns a function approximator (or model) to approximate the query function. In this step, NeuroDB uses solved query instances from a known algorithm to train a model that specifically answers a particular query type well. The model takes the query instance as an input and outputs an answer, and the training objective is to optimize the model so that its answer is as close to ground truth as possible. Finally, at test time, NeuroDB uses the model to answer the queries efficiently, eliminating both the database and the algorithm it learned from.

We use neural networks as our function approximator. Neural networks can learn patterns in the real-world data and the relationship between query input and output, which means small models can answer queries well. They can be trained for specific query distributions, which allows more accurate modeling for the distribution and avoiding redundancies. In fact, NeuroDB can be seen as an approximate result materialization technique, where regions with higher probability in the query space are materialized more accurately. Furthermore, neural networks' architecture can be adjusted to learn complex queries and thus they can be applied to different domains with varying difficulty. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction. %Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section
%The neural network then can be used to replace the database for answering the queries. Our framework is simple and query-type agnostic, that is, it makes no assumption about the query type learned, and yet can provide orders of magnitude performance gains for the specific queries. We use neural networks to be able to capture the complex relationships that can exist between query inputs and outputs. 
However, designing a neural network architecture that can be easily trained, can answer the queries fast and accurately, and can scale with dimensionality and data size is not straightforward. We propose a novel architecture that achieves all of these objectives. 


Overall, NeuroDB offers significant improvements over the state-of-the-art query processing algorithms in multiple aspects. First, we experimentally observed that NeuroDB can answer queries multiple orders of magnitude faster than state-of-the-art and with better accuracy. Thus, in traditional data management systems, NeuroDB can be an addition to the query processing engine and can considerably improve the performance of range aggregate queries. A default query processing engine can answer queries for which NeuroDB is not trained while NeuroDB can be trained for common range aggregate queries, providing substantial improvements for the performance of the system. Furthermore, NeuroDB trained for a specific query is typically much smaller than data size, while the model learned can be used to answer the query it was trained for without accessing the data. This can be beneficial for applications requiring efficient release and storage of data. For instance, location data aggregators (e.g., SafeGraph \cite{safegraph}) can train a NeuroDB to answer the average visit duration query, and release it to interested parties instead of the entire dataset, which can improve the storage, transmission and query processing costs for all parties involved. 

%From another perspective, NeuroDB can be seen as an approximate result materialization technique that takes advantage of query and data distribution to minimize the approximation error. Roughly speaking, regions with higher probability in the query space are materialized more accurately, allowing the framework to perform well for high-dimensional data such as images where queries can be seen as belonging to low dimensional manifolds \cite{roweis2000nonlinear, chen2018sparse}. Intuitively, NeuroDB can be thought of as \textit{memorizing the data points} in the model weights. Although no general guarantee exists that this memorization should take less space than the actual data, in practice, we observe that due to the existence of patterns in the data and the relationship between query input and output, NeuroDB can answer queries by only taking up a fraction of the data size (and without the need to access the database). We note that this is different from merely \textit{memorizing or caching the answers to query points} in the training set, as we experimentally show that NeuroDB learns generalizable patterns between query input and output.

%Overall, in a database system, the choice of what range aggregate queries NeuroDB should be trained to answer is akin to the question of which attributes should be indexed.   


\subsection{Beyond Range Aggregate Queries}
Our observation that queries are functions that can be approximated is not specific to range aggregate queries, and is in fact true for any query type. Considering such representation opens the path for using learned function approximators for answering different database query types. In doing so, an important open question is to understand which function approximators are useful for which query types. 

We take the first step in studying this problem by applying NeuroDB to one more query type. This is possible because NeuroDB framework is query-type agnostic, that is, it does not make assumptions about the query type during training% and only requires solved instances of the query
. We considered two variants of $k$-th nearest neighbour queries. First, we considered $k$-th nearest neighbour queries ($k$-NN), which can be seen as functions that take a $d$-dimensional point as an input, where $d$ is the dimensionality of the database, and output another $d$-dimensional point. Applying NeuroDB to this query type, we experimentally observed that answering such a query requires very large neural networks, which does not provide any benefit in terms of query or storage cost compared with existing methods. Second, we considered the \textit{distance to} $k$-th nearest neighbour query, where the query answer is the distance to and not the actual point in the database. This query is a function that takes a $d$-dimensional query point as an input and outputs a real number. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (for instance, it can be used as a diversity score for selecting samples for training a model) or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. 

We observed that NeuroDB is able to answer distance to $k$-NN queries orders of magnitude faster than state-of-the-art, while only taking space that is a small fraction of data size. NeuroDB achieves this because it answers distance to $k$-NN queries without calculating any distances or finding any of the neighbours at query time. Contrasting this with existing methods that need to find the $k$-th nearest neighbour to calculate distance to $k$-th nearest neighbour shows another advantage of NeuroDB, where it can provide answers for specific queries without unnecessary precomputations. Furthermore, NeuroDB avoids curse of dimensionaity by utilizing the query distribution. For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all potential queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because the space of potential queries can be a small proportion of the total high dimensional space (e.g. for images). %This is in contrast to .  (e.g., finding the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. %without Although distance to $k$-NN queries is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

Overall, we conjecture that NeuroDB is useful for queries that are similar to range aggregate queries and distance to $k$-th nearest neighbour queries, where the answer to the queries is a numerical statistic calculated over the database. We consider studying this conjecture to be an interesting future research direction, where a generic framework can be used to answer multiple different query types. This paper is a first step in that direction, where a framework designed for range aggregate queries is shown to also efficiently answer distance to the $k$-th nearest neighbour queries and outperform the stat-of-the-art for both of them. Although NeuroDB outperforming the state-of the-art in either of the two query types is significant on its own, this paper also sheds light on the possibility that a learned framework can not only be useful for a specific query type, but can be generalizable to multiple query types (specifically query types that are traditionally studied separately, e.g., nearest neighbour queries and range aggregate queries). As such, it can improve the performance of a system while also saving time when designing it.


%The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%Searching the algorithm space translates into searching for good parameters of (or, in other words, learning) a function approximator. In this paper, as an initial attempt, we restrict the algorithm space to the set of parameters of a neural network because it can be searched efficiently. Therefore, we formalize the problem of using learned function approximators to answer database queries and show that, for the specific query types of distance to nearest neighbour query and range aggregate query, a learned neural network can provide better time/space/accuracy trade-offs than existing methods in practice. This, together with the expectation that the performance and availability of hardware for performing matrix multiplication (used in neural network forward passes) will improve in the future  \cite{kraska2018case} suggest using neural networks to answer database queries as a promising research direction.%Intuitive reasons for why a learned neural network can outperform combinatorial methods, whose advantages are detailed in the remained of this section


%Although the NeuroDB framework is query-type agnostic, and as such, can be applied to any query type, in this paper, we only show that it specifically provides orders of magnitude improvement for range aggregate queries and distance to nearest neighbour query. We do not make any claim about its efficiency for other query type. However, due to its good performance for the considered query types, we conjecture that NeuroDB can also be applied to other query types efficiently, but we leave studying this claim for the future work. Nevertheless, both queries considered in this paper are important building blocks of many real-world systems. Distance to nearest neighbour query is useful for various applications such as active learning \cite{settles2009active, fujii1999selective, xu2007incorporating} (for instance, it can be used as a diversity score for selecting samples for training a model) or outlier detection \cite{chandola2009anomaly}, where we are only interested in finding the distance to the $k$-th nearest neighbour and not the $k$-th nearest neighbour itself. Although it is frequently used in various applications, we are unaware of any work that is able to calculate distance to the nearest neighbour accurately for a query without finding any of its nearest neighbours or performing any distance calculation.  

%\noindent\textbf{NeuroDB vs. Combinatorial Methods}. To contrast NeuroDB with existing combinatorial methods, we note that (1) NeuroDB avoids curse of dimensionaity by utilizing the query distribution. For instance, comparing NeuroDB with Voronoi diagrams, Vornoi diagrams materialize the query result for all potential queries exactly, which becomes impractical for high dimensional data. However, this can be redundant, because the space of potential queries can be a small proportion of the total high dimensional space (e.g. for images). (2) NeuroDB can provide answers for specific queries without unnecessary precomputations. For instance, a model can be trained to find the distance to the $k$-th nearest neighbour, without ever finding any of the $k$ nearest neighbours or their distances to the query point. 
%(3) Parallelization of NeuroDB is the problem of performing a forward pass of a neural network in parallel, is a well-studied problem [XX] and does not depend on the query type. 
%(3) NeuroDB uses query and data distribution to learn patterns that allow for answering queries faster. (4) The same framework can be applied to both range aggregate queries and distance to nearest neighbour query, blurring the boundaries between the queries that are traditionally studied separately.


%\noindent\textbf{NeuroDB vs. Machine Learning Methods}. Machine learning methods have been used to solve various combinatorial problems such as TSP, Max cut, etc \cite{li2018combinatorial, khalil2017learning, nazari2018reinforcement}. This paper extends those works to answering generic database queries using neural networks. Answering specific database queries using machine learning has been studied in the literature, such as for indexing \cite{kraska2018case, galakatos2018tree, ding2019alex} and specific aggregate queries \cite{hilprecht2019deepdb, ma2019dbest}. These methods have shown promise in the area they have been applied to, with their success being attributed to the ability of the models to learn and utilize the data and/or query distributions. The main observation in these bodies of work is that a certain database operation (e.g. getting the location a record is stored  for the case of indexing in \cite{kraska2018case}) can be replaced by a learned model. In this paper, we observe the overarching idea that, in fact, answering \textit{any} query can be done by a model, since any query is a function that can be approximated. Using this observation, we show that small, multi-layer neural networks can efficiently and accurately answer range aggregate queries and distance to nearest neighbour queries, improving on the modeling choices of the previous work and the state-of-the-art in the studied query types. %In this respect, our work can be seen as a generalization of the recent work in this area. The advantage in our framework is that it can be applied to different query types. %. However, no framework has been proposed that is able to answer different query types, i.e., both nearest neighbour and range aggregate queries efficiently. Furthermore the proposed techniques use basic regression models [X], while we show how the expressive power of multi-layer neural networks can be utilized.


\subsection{Contributions and Roadmap}

In this paper, we 

\begin{itemize}
        \item Formulate the problem of learning range aggregate queries with function approximators (Sec. \ref{sec:def}); 
        \item Propose the first neural network framework to answer range aggregate queries efficiently  (Sec. \ref{sec:NeuroDB}); and
        \item Show that the same framework can answer distance to nearest neighbour queries (Sec. \ref{sec:NN}).
        \item Our experiments show that
        \begin{enumerate}
            \item {NeuroDB} enjoys orders of magnitude gain in query time and provide better accuracy over state-of-the-art for answering range aggregate queries using real-world, TPC-benchmark and synthetic datasets (Sec.~\ref{sec:exp:rang_agg}); and
            \item The same architecture can be used to answer distance to nearest neighbour query with orders of magnitude gain in query time over state-of-the-art and optimal algorithms on real datasets. NeuroDB's query time is not affected by $k$ and only marginally impacted by data size and dimensionality (Sec. \ref{sec:exp:dist_NN}).
            %\item As a byproduct, we show that {NeuroDB} can learn patterns in the data, and thus is useful for feature learning or when there is missing data (Sec. \ref{sec:exp:NN}).  
        \end{enumerate}

\end{itemize}

We discuss the related work in Sec. \ref{sec:related_work} and further discuss the potentials and limitations of the proposed framework in Sec. \ref{sec:conclusion}. 

%Thus, our method is not applicable for NP-hard queries where collecting samples is difficult. 

%State the problem we're trying to solve: fast solution/not a lot of updates/low dimensional answer. Other examples of low dimensional query

\if 0

\begin{itemize}
    \item \textbf{Motivation}
    \begin{enumerate}
        \item Need for fast query processing, can sacrifice accuracy
        \begin{itemize}
        \item Running Examples: 
        \item (Distance to nearest neighbour query): distance-based outlier detection in video streams, or selecting video frames that are different enough from current samples for training. Want to analyze fast enough to process the stream on the fly
        \item (Range aggregate queries): Calculating avg. pollution level over time and regions for city planing \cite{ma2019dbest}. Large dataset, so exact solution takes too long, but error is acceptable
        \end{itemize}
        \item A lot of Human time is spent on designing efficient algorithms to answer queries
        \begin{itemize}
            \item Example: Different algorithms are designed for answering nearest neighbour queries, range aggregate queries, skyline queries, etc. 
            \item The algorithms are specific to queries
            \item So need to spend a lot of time designing new algorithms for new queries 
        \end{itemize}
    \end{enumerate}
        \item \textbf{Existing Solutions}
        \begin{itemize}
            \item Combinatorial Methods: Calculate answers by an algorithm that accesses the data
            \begin{itemize}
                \item Curse of dimensionality
                \begin{itemize}
                    \item Performance degrades with dimensionality
                    \item Neural network based dimensionality reduction methods are often used
                \end{itemize}
                \item Unnecessary calculations
                \begin{itemize}
                    \item We might only need distance to 100-th nearest neighbour (e.g. for distance based outlier detection), but need to find all the 100 nearest neighbours
                \end{itemize}
                \item Hard to parallelalize
                \item Combinatorial solutions aren't general
                \begin{itemize}
                    \item Hard/time-consuming to design new fast combinatorial method for new queries, or automate the process of designing algorithms
                    \item No combinatorial method can handle \textit{all} queries fast
                \end{itemize}
            \end{itemize}
            \item Learning-based methods
            \begin{itemize}
                \item Have been successfully applied to some database/combinatorial problems
                \item But no general neural network-based framework for learning
            \end{itemize}
        \end{itemize}


    \item \textbf{Neural Databases}
    \begin{itemize}
        \item Overview
        \begin{itemize}
            \item Database queries are functions
            \item Learn from sample queries and their answer
            \item Answer queries without data access
        \end{itemize}
        \item General method for answering any query approximately
        \item Takes advantage of data/query distribution
        \item Can be applied to any query
        \begin{itemize}
            \item The framework is general, but we show that it can be applied to queries with low-dimensional outputs
            \item higher-dimensional output needs more training samples to avoid over-fitting so are harder to learn
        \end{itemize}
        \item Scales easily with more computational power
        \item Differentiable database operations (possible applications in ML)
    \end{itemize}
    \item Neural Database vs. ML for combinatorial optimization
    \begin{itemize}
        \item Answers different queries on a particular database, compared with answering different instances of a problem type
    \end{itemize}
    \item Neural Database vs. existing ML use-cases for DB problems
    \begin{itemize}
        \item Ad-hoc ML use-cases, no general framework applicable to all problems
        \item Indexing \cite{kraska2018case} and aggregate queries \cite{ma2019dbest} are special cases
    \end{itemize}
    \item Contributions
    \begin{itemize}
        \item View of database queries as functions that can be learned
        \item Propose first general framework to answer queries efficiently using neural networks
        \item Design a model based on the framework
        \item Show how it can be applied to nearest neighbour/distance to nearest neighbour/range aggregate queries
        \item Experimentally show it does better than existing methods
    \end{itemize}
\end{itemize}

\fi

==> NeuroDB-ICDE (tech)/NN_queries.tex <==
\begin{figure}
    \centering
    %\hspace*{-cm}
    %\begin{minipage}{0.3\textwidth}
    %\includegraphics[width=\textwidth]{KeyValueStore.eps}
    %\caption{Look-up in Key Value Stores}
    %\label{fig:keyval}
    %\end{minipage}
    %\hfill
    \begin{minipage}{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/NN_points.eps}
    %\caption{Nearest Neighbour Query}
    %\label{fig:NN}
    \end{minipage}
    \hfill
    \begin{minipage}{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/range_count_points.eps}
    %\caption{Range Agg. Query}
    %\label{fig:DistNN}
    \end{minipage}
    \caption{Nearest neighbour, $f_D^1(q)$, distance to nearest neighbour, $f_D^2(q)$, (left) and range aggregate, $f_D^3(q)$, (right) query functions}
    \label{fig:query_functions}
\end{figure}


\section{NeuroDB for Nearest Neighbour Queries}\label{sec:NN}
In this section, we show how the NeuroDB framework can applied to nearest neighbour queries. As discussed in Sec.~\ref{sec:raq_extension}, NeuroDB framework is query type agnostic, and to apply NeuroDB to a query type, it is only required that the query type is represented by query functions. Thus, below we discuss the query representation for two variants of nearest neighbour queries. After specifying the query representation, NeuroDB can readily be applied to answer the queries. 
%Our observation that queries are functions that can be approximated is not specific to RAQs. In fact, any database query can be seen as a function, $f_D(q)$, mapping a query space to some output space. The query space is the set of all the possible inputs to the query and the output space the set of all possible answers to it. For instance, for the nearest neighbour query on a $d$-dimensional database the query space is all the points in $R^d$ and output space is all the points in the database. Algorithms can be seen as functions approximating the query function, or, in other words, as function approximators. . 

%Considering this representation of queries, we can see that Problem \ref{prob:RAQ} is not specific to RAQs, but is the problem of learning any database query. Furthermore, our NeuroDB framework presented in Sec. \ref{sec:NeuroDB} is query-type agnostic, that is, it does not make any assumption about the query function as further discussed in Sec.~\ref{sec:nn:apply} below. Although we do not make any claims about performance of NeuroDB for generic query functions, we take the first step in studying it by applying our framework, designed for RAQs, to answer two nearest neighbour query variants. A significance of this study is that a single framework is used to answer two query types that are traditionally studied separately and the existing algorithms for answering them are different. We first discuss how nearest neighbour query variants can be represented as a function and then discuss how our framework can be applied to answer them. 

%The only requirement is that the query can be represented as a vector $q$ that can be input to a neural network.  TODO: Somewhere mention this requriement, also the requirement that some algorithms are used to obtain the answers. Maybe specify those  in the problem definition.

%\subsection{Query Representation}\label{sec:nn_representation}
\noindent\textbf{$k$-th nearest neighbour query}. Given a $d$-dimensional database, an integer $k$, and a query point $q\in \mathcal{R}^d$, $k$-th nearest neighbour query is to find the point in $D$ whose distance to $q$ is the $k$-th smallest. For this query, we define $f_D(q):\mathcal{R}^d\rightarrow\mathcal{R}^{d}$ as the query function that takes in a point in $\mathcal{R}^d$ and outputs another point in $\mathcal{R}^d\cap D$. 

For the one dimensional database $D=\{1, 2, 3, 5, 6\}$, Fig.~\ref{fig:query_functions} (left) shows the $k$-th nearest neighbour query function for $k=1$ (Shown as $f_D^1(q)$ in the left figure). Observe that $f_D^1(q)$ is a step function, where the output of $f_D^1(q)$ is always a point in the database. $f_D^1(q)$ is constant over the query inputs whose nearest neighbour is the same, and points of discontinuity occur when the nearest neighbour changes (this happens at the mid-point between consecutive data points, shown by dashed lines in the figure). We have also included Fig. \ref{fig:query_functions} (right) for comparison with an RAQ. In Fig.~\ref{fig:query_functions} (right), we consider the count aggregation function and the range predicate is defined by the query variable $q$, $q\in R$, and predicate function $P_f(q, x)$, where $P_f(q, x)$ is set to 1 if $x>q$ and 0 otherwise (i.e., the query input specifies the beginning of the range and all ranges are of the form $(q, \infty)$).

%We were unable to train NeuroDB to be able to answer $k$-th nearest neighbour query with reasonable accuracy. Nevertheless, we experimentally observed that NeuroDB performs very well for distance to the $k$-th nearest neighbour query. We hypothesize that this is due to $k$-th nearest neighbour queries having high-dimensional output spaces which makes learning more difficult. Thus, we only focus on distance to $k$-th nearest neighbour query in the rest of this paper. Our results on $k$-th nearest neighbour query are presented in our technical report \cite{techreport}. Our technical report also contains a case study on a small dataset for nearest neighbour query to better understand what NeuroDB learns. 

%Defining $\Delta_{f_D}(q, y)=|f_D(q)-y|$, we can study the accuracy of the approximation offered by $\hat{f}_D(q;\theta)$. The figure shows that $\Delta_{f_D}(q, \hat{f}_D(q;\theta))<\delta_0$, $\forall q\in \mathcal{R}$, so $E_{q\sim \mathcal{Q}}[\Delta_{f_D}(q, \hat{f}_D(q))]\leq \delta_0$. However,  $E_{q\sim \mathcal{Q}}[\Delta_{f_D}(q, \hat{f}_D(q))]$ may in fact be much lower than $\delta_0$, depending on the distribution $\mathcal{Q}$. 

\noindent\textbf{Distance to $k$-th nearest neighbour}. In addition to $k$-th nearest neighbour query, we also consider the \textit{distance to the $k$-th nearest neighbour} query. That is, if $p$ is the $k$-th nearest neighbour of a query point $q$, then $f_D(q)=d(p,q)$ for some distance metric, $d(p, q)$. Note that $f_D:\mathcal{R}^d\rightarrow\mathcal{R}$. 
As discussed in Sec.~\ref{sec:intro_NN}, this query function is useful for various application, but has not been traditionally studied separately from the nearest neighbour query, because combinatorial methods use a nearest neighbour algorithms to find the distance to the nearest neighbour. However, using neural networks we can directly calculate distance to the nearest neighbour without ever finding any of the nearest neighbours. 
The red curve in Fig. \ref{fig:query_functions} shows this query for $d=1$ and $k=1$ (on the same database mentioned above). Observe that, in contrast to the nearest neighbour query, this query is continuous. Furthermore, its range is a single real number, as opposed to $\mathcal{R}^{d}$. %We will later see how these features impact learning.

For both $k$-NN and distance to $k$-NN query types, following our framework of query specialization discussed in Sec.~\ref{sec:applying_neurodb}, we define $f_D(q)$ to be the query function for a specific value of $k$. Thus, $k$-NN query type is divided into different query functions, each for a value of $k$. The same discussion as in Sec.~\ref{sec:applying_neurodb} for RAQs applies to $k$-NN and distance to $k$-NN queries, e.g., we can learn NeuroDB for common values of $k$ and a default nearest neighbour algorithm can be used to answer the queries for values of $k$ where no model is learned. 

%\subsection{Applying NeuroDB}\label{sec:nn:apply}




==> NeuroDB-ICDE (tech)/RelatedWorks.tex <==
\section{Related Work}\label{sec:related_work}
Related works can be classified into 3 groups: algorithms for RAQs and nearest neighbour queries and machine learning methods for database queries.



\noindent\textbf{Algorithms for Approximate Query Processing}. Approximate query processing (AQP) has many applications in data analytics, with queries that contain an aggregation function and a selection predicate used to report statistics from the data. Broadly speaking, the methods can be divided into sampling-based methods \cite{hellerstein1997online, agarwal2013blinkdb, chaudhuri2007optimized, park2018verdictdb} and model-based methods \cite{graham2012synopses, schmidt2002propolyne, ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. Sampling-based methods use different sampling strategies  (e.g., uniform sampling, \cite{hellerstein1997online}, stratified sampling \cite{chaudhuri2007optimized, park2018verdictdb}) and answer the queries based on the samples.  Model-based methods develop a model of the data that is used to answer queries. The models can be of the form of histograms, wavelets, data sketches (see \cite{graham2012synopses} for a survey) or regression and density based models \cite{ma2019dbest, thirumuruganathan2019approximate, hilprecht2019deepdb}. Generally, these works follow two steps. First, a model of the data is created. Then, a method is proposed to use these data models to answer the queries. The important difference between these works and ours is that the models are created \textit{based on the database} to answer \textit{specific} queries. That is, a model is created that explains the data, rather than a model that predicts the query answer. For instance, regression and density based models of \cite{ma2019dbest} or the sum-product network of \cite{hilprecht2019deepdb} are models of the data that are created independent of potential queries. We experimentally showed that our modeling choice allows for orders of magnitude performance improvement. Secondly, specific models can answer specific queries, (e.g. \cite{ma2019dbest} answers only COUNT, SUM, AVG, VARIANCE,
STDDEV and PERCENTILE aggregations). However, our framework is query-type agnostic and can be applied to any aggregation function. In this respect, our approach is similar to sampling-based methods that can be applied to any aggregation function and selection predicate. However, sampling-based methods fail to capitalize on patterns available in either data points or query distribution, which results in worse performance. 

\noindent\textbf{Algorithms for Nearest neighbour query}. Nearest neighbour query has been studied for decades in the computer science literature \cite{friedman1975algorithm, guan1992equal, bei1985improvement}, and is a key building block for various applications in machine learning and data analysis \cite{shalev2014understanding, chandola2009anomaly, alfarrarjeh2020class, chen2005robust, yu2020combo}. For various applications, such as similarity search on images, it is important to be able to perform the query fast, a problem that becomes hard to address in high-dimensional spaces \cite{weber1998quantitative, gionis1999similarity, arya1998optimal}. As a result, more recent research has focused on approximate nearest neighbour query \cite{zheng2016lazylsh, huang2015query, wang2018randomized, fu2017fast, zhao2020song}. Generally speaking, all the methods iterate through a set of candidate approximate nearest neighbours and prune the candidate set to find the final nearest neighbours. The algorithms can be categorized into locality-sensitive hashing (LSH) \cite{gionis1999similarity, indyk1998approximate, zheng2016lazylsh, wang2018randomized, huang2015query}, product quantization \cite{jegou2010product, johnson2019billion}, tree-based methods  \cite{arya1998optimal, roussopoulos1995nearest},
and graph-based searching \cite{fu2017fast, hajebi2011fast, zhao2020song}. LSH-based and quantization-based methods map the query point to multiple buckets which are expected to contain similar points. %Tree methods partition the space or group the data points using a tree structure and traverse the tree by considering the distance between the query points and the tree nodes. Graph-based methods search the points in an order defined by a graph. The challenge in all the approaches is finding a small enough candidate set, without exponential preprocessing time and memory (Voronoi diagrams can do this but require exponential preprocessing time and memory).

Finding a small candidate set is difficult, and as dimensionality increases more candidate points need to be checked. However, our NeuroDB framework avoids accessing points altogether, and learns a function based on the data that can answer the queries accurately. Moreover, the size of the candidate set increases with $k$, for all the algorithms. That is, more points need to be searched when $k$ increases. However, in an application which only requires distance to the $k$-th nearest neighbour, NeuroDB can directly output the answer, without the value of $k$ affecting query time. We are unaware of any other work that studies distance to $k$-th nearest neighbour without finding any of the nearest neighbours.

\noindent\textbf{Machine Learning for Databases}. There has been a recent trend to replace different database components with learned models \cite{ortiz2018learning, hashemi2018learning, hilprecht2019deepdb, macke2018lifting, nathan2020learning, idreos2019learningb, idreos2019Learninga, kraska2019sagedb, mitzenmacher2018model, ma2019dbest, thirumuruganathan2019approximate, galakatos2018tree, galakatos2018tree}. Most of the effort has been in either indexing (on one dimensional indexes are studied in \cite{kraska2018case, galakatos2018tree, ding2019alex}, with extensions to multiple dimensions studied in \cite{nathan2020learning}, using Bloom filters in \cite{mitzenmacher2018model, macke2018lifting} and key-value stores in \cite{idreos2019learningb, idreos2019Learninga}) or approximate query processing (learning data distribution with a model \cite{thirumuruganathan2019approximate}, using reinforcement learning for query processing \cite{ortiz2018learning}, learning models based on the data to answer queries\cite{hilprecht2019deepdb, ma2019dbest} and cardinality estimation \cite{kipf2018learned, wu2021unified}) with \cite{kraska2019sagedb} discussing how they can be put together to design a database system. The main observation in these bodies of work is that a certain database operation (e.g. retrieving the location of a record for the case of indexing in \cite{kraska2018case}) can be replaced by a learned model. In our paper, we observe the overarching idea that answering \textit{any} query can be performed by a model, since any query is a function that can be approximated. In this respect, our work can be seen as a generalization of the recent work in this area. Solving this more general problem requires a learning method with strong representation power, which motivates our use of neural networks. This is in contrast with simpler models used in \cite{kraska2018case, kraska2019sagedb, ma2019dbest}. %We further note that machine learning has been used to solve various combinatorial optimization problems \cite{li2018combinatorial, khalil2017learning, nazari2018reinforcement}, but we are unaware of any work that considers performing different queries on the same database. We furthermore mention that for many database queries polynomial-time exact solutions exist, that makes sample collection easier, compared with solving NP-hard combinatorial optimization problems. % Generally speaking, these studies assume that the optimization problem is sampled from some distribution, and the goal is to design heuristics that work well for that particular distribution of problems. Various problems such as Travelling Salesman Problem \cite{bello2016neural, khalil2017learning}, Vehicle Routing Problem \cite{nazari2018reinforcement} and other graph optimization problems \cite{khalil2017learning} have been studied. The approaches forgo worst-case approximation guarantees for better empirical approximation in practice. One difference between our work with the abovementioned works is that a database query depends on an input and a database, while the above problems output an answer only based on the input. Although the combinatorial problems can also be formulated as database queries (e.g. a TSP problem can be formulated over some points in a database, with the query being the starting point), 


%.  use machine machine learning methods in databases. There has been recent interest in the database community to replace traditional index structures with learned models \cite{galakatos2018tree, kraska2018case, ding2019alex}. These approaches see an index as a mapping from the query point to a location where the data is stored, and aim at using a function approximator to learn this mapping, instead of using a traditional index. Our work can be seen as a generalization of this idea, where not only an index search, but any database query is seen as a mapping that can be approximated. There has also been work on optimizing queries processing \cite{thirumuruganathan2019approximate, ortiz2018learning} in databases using machine learning. Learning access pattern \cite{hashemi2018learning}. Learning Bloom filters \cite{mitzenmacher2018model}. AQP date driven model \cite{hilprecht2019deepdb}




==> NeuroDB-ICDE (tech)/general_RAQ.tex <==
\section{NeuroDB for General RAQs}\label{sec:raq_extension}
To train NeuroDB, we require a query function $f_D(.)$ and a query set $Q$. NeuroDB treats the query function as a black box, only utilizing it to collect the labels for training samples in $Q$. Thus, we call NeuroDB a \textit{query-type agnostic} framework. Subsequently, after NeuroDB is trained for a query function, it can be used to answer corresponding query instances. As such, to extend NeuroDB to other RAQs, we only need to show how they can be represented as a query function. After such a query function representation is created, we can learn NeuroDB to answer the corresponding query instances. Below, we first discuss how this representation can be obtained in general RAQ settings, then we discuss how NeuroDB can be applied to answer RAQs in real-world databases. 
%To see this, observe that the model training step only utilizes query specific information in Alg.~\ref{alg:get_index} line \ref{alg:get_index:train}, where for each query sample, $q\in Q$, the corresponding true answer, $f_D(q)$, is calculated for training. Furthermore, after the training processes, for any query function, our method for answering queries, depicted in Alg~\ref{alg:get_answer}, is the same as before, and consists of traversing the kd-tree and a forward pass of the neural network. 


%Clearly, for nearest neighbour queries, the method for getting the true answer $f_D(q)$ for training will be different from RAQs, but after training pairs, $(q, f_D(q))$, are collected, the training process and the loss function are the same. 




%\noindent\textbf{Different $AGG$ and $X_m$}. So far, we have discussed how to learn a model to answer a query for a specific aggregation function, $AGG$, and measure attribute, $X_m$. It is easy to see that any specific $AGG$ and $m$ pair define a query function, for which our framework can be used to learn a model. 

\subsection{Query Representation}
\noindent\textbf{General RAQs}. First, we generalize our definition of RAQs. An RAQ consists of a range predicate, and an aggregation function $AGG$. We consider range predicates that can be represented by a \textit{query instance} $q$, a $d_{pred}$ dimensional vector, and a binary \textit{predicate function}, $P_f(q, x)$, that takes as inputs a point in the database, $x$, $x\in D$, and the query instance $q$, and outputs whether $x$ matches the predicate or not. Furthermore, $AGG$ is a function that takes the set of matching data points to the query as an input and outputs a real number. Note that the notion of a measure attribute is implicitly captured in the definition of aggregation function (e.g., $AVG(X_m)$ can be defined by the aggregation function $AGG(S) = \sum_{s\in S}\frac{s[X_m]}{|S|}$, where $s[X_m]$ is the value of $X_m$ attribute for a record $s$). Then, given a predicate function and an aggregation function, range aggregate queries can be represented by the query function $f_D(q)=AGG(\{x|x \in D, p(x, q)=1\})$. 


The above formulation divides the set of all possible RAQs into a set of different query functions, each defined for a specific aggregation and predicate function. In a real-world application, relevant query functions can be created from the query workload, where RAQs with the same predicate and aggregation function but different query instances can be used to define a query function. We avoid specifying how the predicate function should be defined to keep our discussion generic to arbitrary predicate functions, but some examples follow. To represent the RAQs of the form discussed in Sec.~\ref{sec:def}, $q$ can be defined as lower and upper bounds on the attributes and $P_f(q, x)$ defined as the WHERE clause in Sec.~\ref{sec:def}. We can also have $P_f(q, x) = x[1]>x[0]\times q[0]+q[1]$, so that $P_f(q, x)$ and $q$ define a half-space above a line specified by $q$. Furthermore, for many applications, WHERE clauses in SQL queries are written in a parametric form \cite{sql_microsoft, sql_nodepostgres, sql_dataworld}  (e.g., WHERE $X_1> ?param1$ OR $X_2> ?param2$, where $?param$ is the common SQL syntax for parameters in a query). Such SQL queries can readily be represented as query functions by setting $q$ to be the parameters of the WHERE clause. %For instance, a query function can correspond to average over rectangular ranges, while another query function can be for count over half-spaces. Then, considering any such query function, our framework can be applied to learn the query function without any further adjustments. 

%Assuming $\mathcal{D}$ is the domain of our dataset (e.g., $\mathcal{D}=\mathcal{R}^d$ for numerical datasets), $P$ defines a subset of $\mathcal{D}$. A data point, $x\in D$ matches the query if $x\in P$.  Specifically, the answer to a range aggregate query defined by $AGG$ and $P$ is $AGG(\{x|x \in D\cap P\})$. %Many range predicates in the real world have parametric representations. That is, they 





%In practice, they can be created based on the WHERE clause of SQL queries (e.g., for attributes X and Y, and the clause WHERE X between L\_1 and U or Y>L\_2 we define $q$=(L\_1, U, L\_2)). Note that the range predicate can be on any subset of the attributes in the database, and there does not need to be a specific relationship between $d$ and $d_{pred}$.

%For many applications, common range predicates in  RAQs correspond to the same predicate function but with different query variables. For instance, in our geo-spatial database example, the query of average visit duration given a rectangular range is asked for different rectangle locations, which can be specified by a query variable. For such applications, the aggregation function and predicate function are decided in advance (e.g., by system designer), and at query time, the query variable is presented by the user. 



\noindent\textbf{Join and Group By Clauses}. Finally, although answering arbitrary SQL queries is not the focus of this papers, we discuss how RAQs with Join and Group By clauses can also be represented as query functions. If an SQL statement contains Join of tables, we can consider the dataset, $D$, on which the query function is defined to be the Joined tables. Then, the query function can be defined the same way as before, but operating on the joined tables. Furthermore, answering RAQs with a Group By clause using NeuroDB can be done similar to \cite{ma2019dbest}. Consider an RAQ with predicate function $P_f(q, x)$ and with the clause Group By G, where G is an attribute that takes one of $g_1$, ..., $g_k$ values. Such a query can be treated as $k$ different query functions (for each a different model can be learn) where the range predicate for the $i$-th query function, $P_f^i(q, x)$, is defined as $P_f(q, x)\land x[G]==g_i$. 

\subsection{Applying NeuroDB}\label{sec:applying_neurodb}
In our approach, possible RAQs on a database are divided into various query function. Subsequently, we learn different models for different query functions. We call this \textit{query specialization}, where specialized models are trained to answer specific query functions. This is beneficial because, as shown in our experiments, \textit{small specialized models} can answer a query function within microseconds, when the state-of-the-art \textit{non-specialized models} take milliseconds. Intuitively, this huge advantage is due to a specialized model being able to divert all its capacity to learn patterns for a specific query function. 

When a system requires answers to  multiple query functions, the choice of which query functions to learn a model for can be done by the database administrator, akin to the choice of which attribute to index. Intuitively, models should be learned for queries that are frequently performed on the database. Similar to existing work \cite{park2018verdictdb, ma2019dbest}, if a model has not been learned for a particular query function, we assume that a default query processing engine can answer the query. Overall, Learning a model for a query function increases space consumption (for model storage) but improves query time (since learned models can answer a query faster). Given that, in our approach, models take space equal to only a fraction of data size but speed up query time by orders of magnitude, learning multiple models to efficiently answer different query functions proves to be a realistic and beneficial choice. 

Furthermore, in contrast to recent learning-based methods \cite{hilprecht2019deepdb, ma2019dbest}, our approach can learn to answer different RAQs without making assumptions about the query function (besides the fact that the range predicate can be represented by a predicate function). This allows learning arbitrary and potentially application specific RAQs that generic database systems aren't optimized for (e.g., an arbitrary aggregation function on a polygon-shaped range predicate), and can substantially improve the performance of such systems. 

